Short Message Service (SMS) Phishing Attacks and Defenses: A Systematic Review

SMS Phishing (also known as 'smishing') is a growing deceptive social engineering (SE) attack that leverages mobile SMS to conduct cybercrimes such as stealing sensitive information or spreading malware by tricking users into interacting with attackers' messages (e.g., responding to or clicking URLs). This threat has increased rapidly in recent years, causing $470M in financial losses for United States users in 2024 alone. This threat is also evolving rapidly, meaning that attackers continually adapt their tactics, reshaping the landscape. There is a significant body of literature on investigating smishing attacks and defenses. However, there is no systematic review that reflects the current attack and defense landscape along with available resources (i.e., relevant datasets). This motivates us to systematize the current smishing research efforts, including the following four research pillars: (a) user perception and susceptibility, (b) attack characterization, (c) defense landscape, and (d) smishing datasets. This leads us to propose novel future research directions towards effectively mitigating smishing attacks.

==> background.tex <==
\footnote{This section needs a figure or two, with real examples, Maraz can work on it to illustrate the problem, you can also create a scenario based image where either smishing results to stealing info or downloading a malware!}
\ignore{Cybersecurity has become an increasingly critical concern in the digital age. Among the countless threats that individuals and organizations face, phishing attacks stand out as pervasive and continuously evolving cyber threats. Phishing involves deceptive techniques aimed at tricking individuals into divulging sensitive information, such as login credentials or financial details. As traditional phishing methods adapt to new technologies, an emerging and particularly insidious variant is SMS-based phishing, commonly known as "smishing". Since everyone uses texts and has phones, scammers can easily trick people with smishing attacks \citep{goel2018smishing}. These attacks often involve sending fraudulent messages that appear legitimate, leading recipients to disclose sensitive information or download malicious content unwittingly.}

{\color{olive}
Recent studies have highlighted the growing prevalence and sophistication of smishing attacks. Nahapetyan et al. \citep{on_phishing_tactics_nahapetyan2023sms} analyzed over 200 million SMS messages and identified 67,991 phishing messages, demonstrating the scale of the problem. Sonowal \citep{sonowal2020detecting} proposed a method for detecting phishing SMS based on multiple correlation algorithms, emphasizing the need for advanced detection techniques. The challenges posed by smishing extend beyond technological solutions, requiring a deeper understanding of human factors and user behavior \citep{mishra2019content}. Clasen et al. \citep{clasen2021friend} investigated recipient identification of SMS-based phishing, highlighting the importance of user awareness and education in combating smishing attacks.}

%As the threat landscape evolves, addressing the challenges posed by smishing becomes imperative for maintaining robust cybersecurity. %This work focuses on providing a nuanced understanding of smishing, examining recent advancements in detection methodologies and exploring the multifaceted nature of the threat. 

The background encompasses the evolution of phishing attacks from email-centric to SMS-based methods, reflecting the adaptability of cyber adversaries. Understanding the context involves recognizing the inherent challenges in combating smishing, which requires a delicate balance between technological solutions and user awareness.

%The selected papers for this survey collectively contribute to building this understanding by presenting diverse perspectives, methodologies, and insights. This article looks at research on smishing to understand why scammers do it, how common it is, and their latest tricks. By explaining this, the article shows why we need to keep finding new ways to stop smishing attacks as they change. 

==> criticalreview-literature.tex <==


% \begin{figure*}
%   \centering
%   \begin{tikzpicture}[>=Stealth, node distance=1.5cm, every node/.style={text width=2.5cm, align=center, rectangle, draw, minimum height=1cm}]

%     % Nodes
%     \node (smishing) {Smishing Research and Detection};
    
%     \node[below=of smishing, yshift=-2.0cm] (study) {Study/Rule Based};
    
%     \node[below=of study, xshift=-1.5cm] (userstudy) {User study};
%     \node[below=of study, xshift=1.5cm] (psychstudy) {Psych Study};
    
%     \node[below=of smishing, xshift=4.5cm, yshift=-0.5cm] (msganalysis) {Message Analysis};
    
%     \node[below=of msganalysis, yshift=-0.5cm] (contentanalysis) {Content Analysis};
    
%     \node[below=of contentanalysis, xshift=-3.5cm, yshift=-1.5cm] (classicml) {Classic ML};
%     \node[below=of contentanalysis, xshift=-0.5cm, yshift=-1.5cm] (deeplearning) {Deep Learning};
    
%     \node[below=of msganalysis, xshift=3.0cm, yshift=-0.5cm] (urlanalysis) {URL Analysis};
    
%     \node[below=of urlanalysis, xshift=-1.5cm] (lexicalfeatures) {Lexical Features};
%     \node[below=of urlanalysis, xshift=1.5cm] (hostfeatures) {Host-based Features};
    
%     \node[below=of smishing, xshift=-4.5cm, yshift=-0.5cm] (modelexplain) {Model Explainability};
    
%     \node[below=of modelexplain, xshift=-1.5cm] (localapprox) {Local Approximations};
%     \node[below=of modelexplain, xshift=1.5cm] (globalimportance) {Global Feature Importance};
    
%     % Arrows
%     \draw[->] (smishing) -- (study);
%     \draw[->] (study) -- (userstudy);
%     \draw[->] (study) -- (psychstudy);
%     \draw[->] (smishing) -- (msganalysis);
%     \draw[->] (msganalysis) -- (contentanalysis);
%     \draw[->] (contentanalysis) -- (classicml);
%     \draw[->] (contentanalysis) -- (deeplearning);
%     \draw[->] (msganalysis) -- (urlanalysis);
%     \draw[->] (urlanalysis) -- (lexicalfeatures);
%     \draw[->] (urlanalysis) -- (hostfeatures);
%     \draw[->] (smishing) -- (modelexplain);
%     \draw[->] (modelexplain) -- (localapprox);
%     \draw[->] (modelexplain) -- (globalimportance);
    
%   \end{tikzpicture}
%   \caption{Smishing research and detection literature category}
%   \label{fig:category_smishing}
% \end{figure*}

This paper highlights the five major research focus areas in smishing literature domain. We also provide critical analysis of existing works, understand the chronology of research, compile available resources, and identify gaps to conduct future research in this domain. Figure \ref{fig:thematic-diagram} presents a tree diagram on the overview of the existing smishing research efforts and focus areas highlighted in this paper.  

\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{Figures/fiq_1.png}
  \caption{Tree diagram presenting the primary focused research areas in SMS phishing}
  \label{fig:thematic-diagram}
\end{figure}

%\footnote{Fig. 1 needs update: `Smishing Attacks' should change to `Threat Landscapes', `Smishing Detection' should change to `Detection Methods', `Smishing Countermeausres' should change to `Defense Countermeasures', add `User Psychological Perception' as a focus area, add `SMS Datasets' as a focus area, deep learning is missing under 'Detection Methods'}



\begin{figure}[!b]
  \centering
  \includegraphics[width=\linewidth]{Figures/Draft_Threat_Landscape.jpg}
  \caption{SMS Phishing Threat Landscape}
  \label{fig:threat-landscape}
\end{figure}


%{\footnote{\color{blue} May be adding a timeline image of history of smishing (Optional)}}
%The literature motivates us towards smishing research and detection techniques into three main approaches:

% \begin{itemize}
%     \item Study/ Rule Based Research works - Analyzes rule based systems, SMS phishing related user studies, psychological patterns with smishing attacks
    
%     \item Content analysis - Analyzes message text using Classical ML and deep learning

%     \item URL analysis - Identifies malicious URLs in messages using lexical or host features

%     \item Model explainability - Generates local or global explanations for model predictions

% \end{itemize}


\subsection{Smishing Threats and Attack Landscapes}


\ignore{
\begin{itemize}
    \item Smishing Attacks - This branch explores the different ways attackers use smishing to achieve their goals.
    
    \item Smishing Detection - This branch examines the various approaches used to identify and prevent smishing attempts.

    \item Smishing countermeasure - This branch outlines the strategies employed to mitigate the risks associated with smishing.

\end{itemize}
}

%We have collected all the indexed articles and papers published in various peer-reviewed journals, conference, workshop proceedings, and posters 
In this focus area, we try to systematically understand the smishing threats, attack types, attack themes and potential impacts trough portraying a landscape. %The prior arts we are discussing in this section follow this tree of research problems and solution methodologies.

\noindent \textbf{Types of Smishing:} We feel smishing threats or attacks can be classified into different types based on diverse factors such as content-based classification, sender information-based classification, target audience-based classification, intent-based classification, message delivery technique-based classification, message topic/theme-based classification, and campaign-size based classification. Next, we deep-dive into each of these classification to understand the various types of smishing messages. 

%In literature we observe the main objective of smishing attacks are stealing sensitive and valuable information, distributing malware/ransomware, and/or gain financial benefits \citep{on_phishing_tactics_nahapetyan2023sms}.

%\noindent Smishing Techniques: Details the manipulative tactics used by attackers to trick victims, like social engineering, urgency creation, and sender spoofing \citep{phishing_comp_study_alkhalil}.
 
 %\noindent Impact of Smishing: Highlights the potential consequences for victims who fall prey to smishing attacks, including financial loss, identity theft, and data breaches \citep{clasen2021friend}.
    \subsubsection{Content-based classification}
    \vspace{-0.25mm}In terms of content diversity, we see smishing messages attached with \textit{malicious URLs}, \textit{malicious files}, \textit{image with embedded links}, \textit{QR codes}, or \textit{pre-texting conversations}. Here, malicious URLs can direct users to a fake website or downloads malicious software (malware or ransomware) onto the mobile device, while malicious attachments included with an SMS may disguise as a legitimate attachment that may infect the device. Next, malicious website links embedded within an image or QR codes can make users fall victim to phishing attacks. Furthermore, the pre-texting can often be used as a conversation starter that can later lead to compromise users and fall prey to their attacks.  
    
    %Social Engineering or Pretexting: Messages exploit trust by impersonating legitimate entities (e.g., banks, service providers, or governmental institutions).
%Example: An SMS claiming an account issue and requesting immediate action.
    \subsubsection{Sender-based classification}
    \vspace{-0.25mm}
    We can also classify smishing threats in terms of sender information such as- \textit{spoofed numbers} that are used imitating legitimate organizations, \textit{short codes} that are used by SMS marketing or advertising, \textit{random numbers} often broadcast to non-targeted audience, and \textit{email address} that can be created algorithmically or for mimicking a legitimate entity.    
    
    \subsubsection{Target audience-based classification}
    When considering the target audience as the classification factor, smishing threats can be classified into \textit{targeted spear-smishing} where specific individuals are targeted based on previous reconnaissance activities and \textit{mass-smishing} where a message is sent to many unknown targets as message broadcast for opportunistic attacks. Usually targeted smishing needs more preparation and sophistication with potentially higher success rates, while the mass smishing is usually less sophisticated to carry on but with lower success rates. 
    
    \subsubsection{Intent-based classification} Based on the intent (or goal) of the attackers, smishing can be classified into \textit{steal information}, \textit{harvest credential}, \textit{financially benefit}, \textit{identity theft}, and \textit{recon for information gathering}. There might be certain intents which can be achieved through subsequent successful smishing attacks with another intent. 
    
    %\subsubsection{Message delivery technique-based classification}
    
    \subsubsection{Theme-based classification}
    The topic or themes within a smishing message can vary to connect users and make them trust the SMS for further interactions. The more relevant the theme is, the higher the chance of a successful attack. From existing literature, we find that Nahapetyan et al. \citep{nahapetyanposter_2023} presents the following themes of smishing campaigns-- \textit{general-theme}, \textit{account-theme}, \textit{financial-theme}, \textit{delivery-theme}, \textit{casino-theme}, \textit{surveys-theme}, \textit{medical-theme}, \textit{Apple-theme}, \textit{download-theme}, \textit{sales-theme}, \textit{loans-theme}, \textit{betting-theme}, \textit{taxes-theme}, and \textit{unknown}. The unknown class is a possibility as new themes may evolve over time that are unique in nature and may not be classified into existing established themes. However, themes can evolve with new events around the globe. To illustrate, COVID-19 has emerged as a theme in early 2020, which was not existing prior to 2019. Furthermore, themes can also be seasonal that would usually correspond to specific timings of the year, while urgency-driven themes such as messages related to some subscription account or missing a product delivery are used as tactics to compromise victims.   
    %\subsubsection{Time-based classification}
    
    \subsubsection{Campaign-size based classification} If size and reach of the smishing campaigns are considered, the smishing can be classified into-- (i) individual message attacks, (ii) single template smishing campaigns, (iii) multiple template single theme large campaigns, and (iv) campaign operations, which are described in detail below. 
    
    \noindent \textbf{Individual attacks:} Sometime, we may encounter with messages that are very unique and does not connect to any known themes, sender information. These attacks may be crafted to send to single user or a very limited number of users and send from a personal phone numbers using manual SMS sends. We can refer these attacks as individual message attacks. These attacks may be conducted using a few rouge sim cards. 

    \noindent \textbf{Single template campaigns:} 
    In this case, attackers would like to reach many users using a single message template and send the same message to multiple receiver phone numbers. 
    
    \noindent \textbf{Multi-tempalte large campaigns:} Oftentimes attackers would create multiple templates of similar themes to send to various diverse target population, usually these campaigns would have multiple templates for attacking various user groups aiming to maximize the number of victims. However, they have a known themes and listed target brands, which would be constant throughout the campaigns. Attack campaigns often leverage automated tools to send out a massive number of text messages simultaneously. Analyzing attacks at campaign-level can reveal patterns in the language, urgency levels, and impersonated sources used by scammers.
    
    \noindent \textbf{Campaign operations:} Some attacks may connect multiple big and small campaigns together using common shared infrastructures, which would be financially more beneficial for the attackers. We can refer these threats as \textit{campaign operations}, indicating a common owner group is running the campaign operations that hosts multiple big smishing campaigns to reach diverse user groups as well as targeting different brands and themes. We believe these operation owners may create new campaigns to generate smishing attacks with new themes to make them more trustworthy to their victims. 
    
    %understanding the common tactics used i individual smishing attacks, users can be better equipped to identify and avoid them. Analyzing the specific content and techniques of individual attacks can provide valuable insights for researchers developing detection methods.
    
    %\subsubsection{Attack Campaigns} Smishing attacks can also be launched in large-scale campaigns, targeting a broad range of phone numbers or specific demographics. Attack campaigns often leverage automated tools to send out a massive number of text messages simultaneously. These campaigns may employ similar tactics across messages, aiming to maximize the number of victims who fall prey to the scam. Analyzing attack campaigns can reveal patterns and trends in the language, urgency levels, and impersonated sources used by scammers. Understanding the scope and characteristics of smishing campaigns is crucial for developing effective detection systems that can identify and block them.

%\footnote{check if this old text needs to be placed somewhere}
%{\color{red}By understanding the various types of smishing attacks (Branch 1), the methods used to detect them (Branch 2), and the available countermeasures (Branch 3), we can effectively combat this growing cybersecurity threat. This comprehensive approach that combines technical detection methods with user awareness and education, alongside law enforcement efforts, strengthens our defenses against smishing scams and protects individuals from potential financial loss and identity theft. Moreover, in table \ref{tab:method_sum} we have shown all the works' methodology according to our thematic organization to show the diversity of the research work we chose to survey.}

    
\subsection{Smishing Detection Methods}
In this section we synthesize articles on various smishinng detection mechanisms using rule-based, ML-based, DL-based, and hybrid approaches. We also try to analyze if explainability and transparency aware models are proposed in existing literature. 

\begin{table*}[!t]
\centering
\caption{Summary Analysis of Existing Smishing Detection Methods}
\label{tab:method_sum}
\resizebox{0.90\textwidth}{!}{\begin{tabular}{c|c|cc|cc|cc}
\toprule
\textbf{Authors and Year} &   \textbf{Method}   &             \multicolumn{2}{|c|}{\textbf{Content Analysis}} &     \multicolumn{2}{|c|}{\textbf{URL Analysis}}& \multicolumn{2}{|c}{\textbf{Model Explainability}} %& \textbf{User Study} 
\\
\midrule
                 - & - & \textbf{Machine Learning} & \textbf{Deep Learning} & \textbf{Lexical Features} & \textbf{Host Features} &     \textbf{SHAP/LIME} & \textbf{Potential} &
\midrule
%NEUPANE et al., 2015 \citep{multi_modal_neupane} &                     . &            . &             . &                . &             . &                    . & . & ✓ \\
%SIDDIQI et al., 2016\citep{a_study_psy_siddiqi} &   . &            . &             . &                ✓ &             . &                    . & . \\
GOEL et al., 2018 \citep{goel2018smishing} & . & ✓ & . & . & . & . & . \\
MISHRA et al., 2019 \citep{mishra2019content} & . & ✓ & . & ✓ & . & . & . \\
GHOURABI et al., 2020 \citep{ghourabi2020hybrid} & . & . & ✓ & . & . & . & . \\
SONOWAL, 2020 \citep{sonowal2020detecting} & . & ✓ & . & . & . & . & ✓ \\
ALKHALIL et al., 2021 \citep{phishing_comp_study_alkhalil} & . & ✓ & . & ✓ & ✓ & . & . \\
BOUKARI et al., 2021 \citep{mldetect_smishing_frauds_boukari} & . & ✓ & . & . & . & . & . \\
GHOURABI et al., 2021 \citep{smdetector_ghourabi} & . & ✓ & ✓ & ✓ & . & . & . \\
% BLANCAFLOR et al., 2021 \citep{blancaflor2021let} &                     . &            . &             . &                . &             . &                    . & . & ✓\\
NJUGUNA et al., 2021 \citep{njuguna2021model} & . & ✓ & . & . & . & . & . \\
% CLASEN et al., 2021 \citep{clasen2021friend} &                     . &            . &             . &                . &             . &                    . & . & ✓\\
ULFATH et al., 2022 \citep{ulfath2022detecting} & . & ✓ & . & . & . & . & . \\
HOSSAIN et al., 2022 \citep{spam_filtering_cnn_lstm_hossain} & . & ✓ & . & . & . & . & . \\
MISHRA et al., 2022 \citep{smishing_detector_security_model_mishra_2020} & . & ✓ & . & ✓ & ✓ & . & . \\
JAIN et al., 2022 \citep{content_url_analysis_jain} & . & ✓ & . & ✓ & . & . & . \\
MISHRA et al., 2022 \citep{implement_smishing_detector_mishra_2022} & . & . & ✓ & ✓ & ✓ & . & . \\
% RAHMAN et al., 2022 \citep{user_really_respond_rahman} &                     . &            . &             . &                . &             . &                    . & . & ✓\\
AKANDE et al., 2023 \citep{smsprotect_akande} & Rule-based & ✓ & . & . & . & . & . \\
EJAZ et al., 2023 \citep{life_long_phsising_ejaz} & . & . & ✓ & ✓ & . & . & . \\
KARHANI et al., 2023 \citep{karhani_phishing_2023} & . & ✓ & . & . & ✓ & . & . \\
MISHRA et al., 2023 \citep{dsmish_mishra_2023} & Rule-based & ✓ & . & . & ✓ & . & . \\
TIMKO et al., 2023 \citep{commerial_anti_smishing_timko_2023} & . & ✓ & . & ✓ & ✓ & . & . \\
NAHAPETYAN et al., 2023 \citep{on_phishing_tactics_nahapetyan2023sms} & . & . & . & ✓ & . & . & . \\
SIDHPURA et al., 2023 \citep{sidhpura2023_fedspam:} & . & . & ✓ & . & . & ✓ & . \\
KANAOKA et al., 2023 \citep{kanaoka2023beyond} & . & . & . & ✓ & . & . & . \\
SEO et al., 2024 \citep{seo2024device} & . & . & ✓ & . & . & . & ✓  \\
Hapase et al., 2024 \citep{hapase2024telecommunication} & . & . & ✓ & ✓ & . & . & . \\

\bottomrule
\end{tabular}}
\end{table*}

\subsubsection{Rule-based approach} 
%Literature on rule-based detection approach highlight  traditional detection methods that rely on predefined rules to flag suspicious messages based on keywords, URLs, or sender patterns .  
Rule-based detection in smishing research represents a traditional approach that relies on pre-defined rules to identify suspicious messages \citep{smsprotect_akande}. These rules target specific characteristics commonly found in smishing attempts.  For example, rules might flag messages containing keywords associated with phishing scams (e.g., "urgent," "account locked"), suspicious URLs with specific patterns, or sender information that appears spoofed or illegitimate. While this method offers a simple and efficient way to catch some smishing attempts, its effectiveness can be limited.  Attackers can adapt their tactics to evade basic rules, and the approach might struggle with nuanced language or entirely new attack formats.

\subsubsection{Machine Learning-based approach} 
%{\color{red}Discusses the use of advanced algorithms (supervised learning, anomaly detection) to analyze messages and identify potential smishing attempts with greater accuracy \citep{commerial_anti_smishing_timko_2023}.}
Beyond rule-based methods, ML based approaches offer a more sophisticated and diverse smishing detection. There are various categories of features that the ML models are depending upon. We highlight the existing literature based on the features used in current ML based detection techniques. 
Classical Machine Learning: This approach utilizes established algorithms like Support Vector Machines (SVMs) or Naive Bayes classifiers. These algorithms are trained on features extracted from message content, such as keywords, part-of-speech patterns, or sentiment analysis.

\noindent\textbf{Leveraged Features or Indicators.} We usually observe URL-based and text content-based features as indicators of smishing attacks. 

\noindent\textbf{(i) Content Features:}
 This section explores how machine learning can be leveraged to analyze the actual content of SMS messages. Machine learning algorithms can learn from large datasets of labeled messages (smishing vs. legitimate) to identify patterns and features that distinguish malicious content. We will delve into two main approaches within Content Analysis:


% A paper by Goel et al. proposes a new system called Smishing-Classifier to detect smishing attacks on mobile phones\citep{goel2018smishing}. Smishing is a type of phishing attack where attackers trick users into revealing personal information through text messages. The system uses a Naive Bayes classifier to analyze the content of SMS messages and identify keywords commonly used in smishing attempts. Since SMS messages are short and informal, the system also applies text normalization techniques to improve feature extraction. The authors claim their system offers an effective way to distinguish between legitimate and smishing messages.

% Mishra et al. proposes a novel content-based approach for detecting smishing attacks on smartphones\citep{mishra2019content}. Smishing is a combination of SMS and phishing, where attackers send text messages with malicious URLs to steal users' sensitive information. The proposed method analyzes both the SMS content and URL behavior to detect smishing attempts. It uses text pre-processing techniques to identify malicious keywords, URLs, phone numbers, and email addresses in the message. Additionally, a machine learning algorithm is employed to classify messages based on malicious keywords. Finally, the system analyzes the URL for signs of malicious behavior, such as the presence of forms or the download of APK files. This combination of techniques helps to reduce false positives compared to existing methods that rely solely on SMS content analysis.

\noindent\textbf{(ii) URL Features:}
While analyzing message content is crucial, smishing attacks often rely on malicious URLs to steal user information or deploy malware. This section explores URL Analysis, a critical technique that examines the URLs embedded within suspicious messages. By dissecting these URLs, we can extract valuable clues that point to their legitimacy or malicious intent. We will focus on two key types of features used for URL Analysis:
\begin{itemize}
    \item URL Lexical information: This approach focuses on the analysis of the URL structure itself. Features like unusual characters, excessive length, presence of subdomains, or specific keyword patterns within the URL can indicate potential red flags.
    
    \item URL Host information:  Here, the focus shifts to analyzing the website or server associated with the URL. Techniques involve checking the website's reputation, age, and registration details. Additionally, analyzing the website content itself for phishing elements or malware presence can further strengthen the detection process.
\end{itemize}

%-------- Comparison table 1 ----------------------%
\begin{table*}[!ht]
\caption{Critical Analysis of Smishing Detection Literature}
\label{tab:review-1}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Reference} & \textbf{Key Idea} & \textbf{Strengths} & \textbf{Weaknesses} \\

%& \textbf{Reference} \\ 
\hline

\multicolumn{1}{|p{5em}|}{SHINDE et al., 2024\citep{shinde2024sms}} &
\multicolumn{1}{p{17em}|}{OCR-based detection, hybrid model approach and user-centric application} & 
\multicolumn{1}{p{17em}|}{94.13\% accuracy, the web app allows users to detect spam from screenshots and adaptability in detection} & 
\multicolumn{1}{p{17em}|}{Scalability limitations, retraining requirements and retraining requirements.} \\
%& \multicolumn{1}{p{4em}|}{Seo et al., 2024 \citep{seo2024device}}\\

\hline

\multicolumn{1}{|p{5em}|}{MEHMOOD et al., 2024\citep{mehmood2024enhancing}} &
\multicolumn{1}{p{17em}|}{Deep learning approach using CNN-LSTM, comparison with BiLSTM, GRU and applications in mobile cybersecurity} & 
\multicolumn{1}{p{17em}|}{99.74\% accuracy with high precision, minimizing false positives and comprehensive evaluation.} & 
\multicolumn{1}{p{17em}|}{Potential for overfitting, computational intensity and reliance on data quality} \\
%& \multicolumn{1}{p{4em}|}{Seo et al., 2024 \citep{seo2024device}}\\

\hline

\multicolumn{1}{|p{5em}|}{SEO et al., 2024\citep{seo2024device}} &
\multicolumn{1}{p{17em}|}{Deep learning-based model, text evasion attack defense, accuracy (99\%) using 1.2 million messages dataset.} & 
\multicolumn{1}{p{17em}|}{Real-world data trains on-device, privacy-focused model for SMS spam (0.99 accuracy, lightweight, combats text evasion).} & 
\multicolumn{1}{p{17em}|}{The effectiveness of EVA tools for all types of text evasion attacks might need further exploration.} \\
%& \multicolumn{1}{p{4em}|}{Seo et al., 2024 \citep{seo2024device}}\\
\hline

%\multicolumn{1}{|p{0.4em}}{6} &    
\multicolumn{1}{|p{5em}|}{Neupane et al., 2024 
\citep{multi_modal_neupane}} &
\multicolumn{1}{p{17em}|}{EEG \& eye tracking assess user alertness for future applications. } & 
\multicolumn{1}{p{17em}|}{Tests user behavior \& warns of malware - future in real-time neuro \& eye tracking. } & 
\multicolumn{1}{p{17em}|}{Users miss phishing clues despite focus - low detection accuracy.}\\ 
%& \multicolumn{1}{p{4em}|}{NEUPANE et al, 2015 \citep{multi_modal_neupane}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{11} &    
\multicolumn{1}{|p{5em}|}{MISHRA et al., 2023\citep{dsmish_mishra_2023}} &
\multicolumn{1}{p{17em}|}{SMS phishing targets smartphones - detects URL authenticity \& extracts key features.} & 
\multicolumn{1}{p{17em}|}{Achieves 97.93\% accuracy in detecting phishing attacks, consistent across metrics.} & 
\multicolumn{1}{p{17em}|}{Limited number of features and lack of comparison with other.} \\
%& \multicolumn{1}{p{4em}|}{MISHRA et al, 2023 \citep{dsmish_mishra_2023}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{13} &    
\multicolumn{1}{|p{5em}|}{SIDHPURA et al., 2023 
\citep{sidhpura2023_fedspam:}} &
\multicolumn{1}{p{17em}|}{Federated learning trains on local models, iteratively improves, for final prediction.} & 
\multicolumn{1}{p{17em}|}{DistilBERT (98\% accuracy) predicts spam \& analyzes key words.} & 
\multicolumn{1}{p{17em}|}{Can be susceptible to adversarial attacks. 
} \\
%& \multicolumn{1}{p{4em}|}{SIDHPURA et al, 2023 \citep{sidhpura2023_fedspam:}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{14} &    
\multicolumn{1}{|p{5em}|}{KARHANI et al., 2023\citep{karhani_phishing_2023}} &
\multicolumn{1}{p{17em}|}{SMS phishing detection with SVM. Combines domain \& NLP features to flag malicious sites.} & 
\multicolumn{1}{p{17em}|}{Hybrid machine learning model achieves high accuracy (99.40\%) and F1 score (>99\%) for SMS phishing detection.} & 
\multicolumn{1}{p{17em}|}{Limited to proof of concept without practical tools and unable to handle real-time threats due to time complexity.
} \\
%& \multicolumn{1}{p{4em}|}{KARHANI et al, 2023 \citep{karhani_phishing_2023}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{15} &    
\multicolumn{1}{|p{5em}|}{EJAZ et al., 2023\citep{life_long_phsising_ejaz}} &
\multicolumn{1}{p{17em}|}{Continual learning improves SMS phishing detection (outperforms rules)  with minimal retraining \& thrives on limited data.} & 
\multicolumn{1}{p{17em}|}{SMS phishing defense with continual learning maintains high accuracy (tolerates 2.45\% drop) and minimizes false negatives using EWC.} & 
\multicolumn{1}{p{17em}|}{Traditional VNNs struggle with new phishing tricks (undetected first-time attacks) and lose accuracy in fast-evolving situations.} \\ 
%& \multicolumn{1}{p{4em}|}{EJAZ et al, 2023 \citep{life_long_phsising_ejaz}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{20} &    
\multicolumn{1}{|p{5em}|}{ULFATH et al., 2022\citep{ulfath2022detecting}} &
\multicolumn{1}{p{17em}|}{Uses ML with NLP, employs feature extraction, cccuracy (98.39\%) using SVM} & 
\multicolumn{1}{p{17em}|}{Leverages state-of-the-art ML and NLP techniques, feature selection focused and Reports strong evaluation metrics on a benchmark dataset.} & 
\multicolumn{1}{p{17em}|}{Cutting-edge ML \& NLP (focused features) excel on benchmark data, but lacks details on evolving language \& attack tactics.} \\
%& \multicolumn{1}{p{4em}|}{Ulfath et al., 2022 \citep{ulfath2022detecting}}\\

\hline

\multicolumn{1}{|p{5em}|}{JAIN et al., 2022\citep{content_url_analysis_jain}} &
\multicolumn{1}{p{17em}|}{SMS spam detection: analyzes text \& URLs with TF-IDF for rare words. Trains on two datasets with oversampling.} & 
\multicolumn{1}{p{17em}|}{Authors achieve 99\% accuracy in spam detection with high-quality, filtered data.} & 
\multicolumn{1}{p{17em}|}{Did not checked with the messages without any URLs.} \\

%\multicolumn{1}{|p{0.4em}}{1} &    
%\multicolumn{1}{|p{4em}|}{%On SMS Phishing Tactics and Infrastructure 
%&\multicolumn{1}{p{4em}|}{Nahapetyan et al, 2023 \citep{on_phishing_tactics_nahapetyan2023sms}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{10} &    
\multicolumn{1}{|p{5em}|}{MISHRA et al., 2022\citep{implement_smishing_detector_mishra_2022}} &
\multicolumn{1}{p{17em}|}{Neural net picks best 7 features for smishing SMS detection. } & 
\multicolumn{1}{p{17em}|}{Neural net beats other methods (1.11\%) for smishing with 97.4\% accuracy (URLs at 94\%). } & 
\multicolumn{1}{p{17em}|}{Not explained.} \\
%& \multicolumn{1}{p{4em}|}{MISHRA et al, 2022 \citep{implement_smishing_detector_mishra_2022}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{12} &    
\multicolumn{1}{|p{5em}|}{HOSSAIN et al., 2022\citep{spam_filtering_cnn_lstm_hossain}} &
\multicolumn{1}{p{17em}|}{English spam SMS detection: CNN-LSTM combo with TF-IDF evaluation. } & 
\multicolumn{1}{p{17em}|}{Accuracy 98.40\%, F1-score 98\% and effectiveness of Word-embedding described.} & 
\multicolumn{1}{p{17em}|}{Did not explain the black box CNN-LSTM model
} \\
%& \multicolumn{1}{p{4em}|}{HOSSAIN et al, 2022 \citep{spam_filtering_cnn_lstm_hossain}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{7} &    
\multicolumn{1}{|p{8em}|}{GHOURABI et al., 2021\citep{smdetector_ghourabi}} &
\multicolumn{1}{p{17em}|}{Phishing SMS app: combines URL checks, keywords \& AI to report smishing.} & 
\multicolumn{1}{p{17em}|}{Multilingual BERT works beyond English/Arabic with 99.63\% accuracy. }& 
\multicolumn{1}{p{17em}|}{Defense on adversarial attacks not discussed.} \\ 
%& \multicolumn{1}{p{4em}|}{GHOURABI et al, 2021 \citep{smdetector_ghourabi}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{16} &    
\multicolumn{1}{|p{8em}|}{BOUKARI et al., 2021\citep{mldetect_smishing_frauds_boukari}} &
\multicolumn{1}{p{17em}|}{Phishing SMS tool (Python) stops attacks, analyzes importance of terms (TF-IDF) with demo.} & 
\multicolumn{1}{p{17em}|}{SMS fraud detection app adaptable to vishing \& phishing.} & 
\multicolumn{1}{p{17em}|}{Current AI lacks complete fraud detection (relies on complaints) with low recall \& high false negatives.} \\ 
%& \multicolumn{1}{p{4em}|}{BOUKARI et al, 2021 \citep{mldetect_smishing_frauds_boukari}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{22} &    
\multicolumn{1}{|p{5em}|}{SONOWAL, 2020\citep{sonowal2020detecting}} &
\multicolumn{1}{p{17em}|}{Evaluates rank correlation algorithms for combined classifiers to reduce feature needs.} & 
\multicolumn{1}{p{17em}|}{Focuses on feature selection, explores different correlation algorithms and accuracy 98.40\%} & 
\multicolumn{1}{p{17em}|}{Evaluates rank correlation for combined classifiers (fewer features). Lacks feature details, dataset limitations, and explanation for Kendall's dominance.} \\
%& \multicolumn{1}{p{4em}|}{Sonowal, 2020 \citep{sonowal2020detecting}}\\

\hline

\multicolumn{1}{|p{5em}|}{MISHRA et al., 2020\citep{smishing_detector_security_model_mishra_2020}} &
\multicolumn{1}{p{17em}|}{SMS phishing detector uses 4 modules (text, URL, code, APK) for 96\% accuracy, covering more aspects than others. } & 
\multicolumn{1}{p{17em}|}{Covers more security aspects than others, overall accuracy: 96.29\% and Naive Bayes Classifier accuracy: 91.6\%} & 
\multicolumn{1}{p{17em}|}{Rule-based methods miss new smishing tactics \& URL behavior analysis is lacking.} \\
%& \multicolumn{1}{p{4em}|}{MISHRA et al, 2022 \citep{smishing_detector_security_model_mishra_2020}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{25} &    
\multicolumn{1}{|p{5em}|}{GHOURABI et al., 2020\citep{ghourabi2020hybrid}} &
\multicolumn{1}{p{17em}|}{Arabic \& English SMS spam: CNN-LSTM vs. other ML models.} & 
\multicolumn{1}{p{17em}|}{CNN-LSTM tackles mixed-language (Arabic \& English) SMS spam with 98.37\% accuracy. } & 
\multicolumn{1}{p{17em}|}{Lacks details about the specific features considered by the CNN-LSTM model.} \\
%& \multicolumn{1}{p{4em}|}{Ghourabi et al., 2020 \citep{ghourabi2020hybrid}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{19} &    
\multicolumn{1}{|p{5em}|}{MISHRA et al., 2019\citep{mishra2019content}} &
\multicolumn{1}{p{17em}|}{Mobile smishing detection combines text and URL analysis to lower false positives than prior methods.} & 
\multicolumn{1}{p{15em}|}{Analyzing message content and URL behavior for smishing detection with a focus on reducing false positives.} & 
\multicolumn{1}{p{17em}|}{Relies on keyword lists, limited URL behavior analysis and no mention of specific ML algorithm} \\
%& \multicolumn{1}{p{4em}|}{Mishra et al., 2019 \citep{mishra2019content}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{18} &    
\multicolumn{1}{|p{5em}|}{GOEL et al., 2018\citep{goel2018smishing}} &
\multicolumn{1}{p{17em}|}{Smishing word analysis: normalizes messages and uses Naive Bayes to classify Smishing from regular texts.} & 
\multicolumn{1}{p{17em}|}{Simplicity and Adaptability } & 
\multicolumn{1}{p{17em}|}{Limited Features, Naive Bayes limitations  and no evaluation.} \\
%& \multicolumn{1}{p{4em}|}{Goel et al., 2018 \citep{goel2018smishing}}\\

\hline


% by Mostaq: Not smashing detection related paper 
% %\multicolumn{1}{|p{0.4em}}{5} &    
% \multicolumn{1}{|p{5em}|}{%A Study on the Psychology of Social Engineering-Based Cyberattacks and Existing Countermeasures
% \citep{a_study_psy_siddiqi}} &
% \multicolumn{1}{p{17em}|}{{\color{red}In-depth analysis of Social engineering attack tactics.}} & 
% \multicolumn{1}{p{17em}|}{Provides an detail analysis of Social engineering-based cyberattacks.} & 
% \multicolumn{1}{p{17em}|}{The mapping might not represent every age group or human behavior.
% } \\ 
% %& \multicolumn{1}{p{4em}|}{SIDDIQI et al., 2022 \citep{a_study_psy_siddiqi}}\\

% \hline




\end{tabular}
}
\end{table*}

\subsubsection{Deep Learning-based approach}
In recent years, Deep Learning techniques have shown promising results in content analysis. Deep neural networks, with their ability to learn complex relationships from data, can be particularly effective in identifying nuanced language patterns and uncovering hidden features within message content that might be missed by classical machine learning approaches.

\subsubsection{Natural language processing-based approach}
Different strategies that would integrate NLP technologies and machine learning algorithms to investigate fake content are used. The model combining TF-IDF with LDA was shown to surpass the performance of Weight Average Word2Vec \citep{samad2023smishguard} in terms of accuracy and F1 score, indicating that the information provided by text analysis is of value in this domain. Random Forest and Extreme Gradient Boosting were the machine-learning methods that the researchers preferred. These two models performed very well in detecting smishing attacks, further consolidating the versatility of such approaches to deal with such challenges. These approaches provided an F1 score of over 94\% and proved their value in practical situations \citep{chen2023using}. Combining NLP with machine learning provides substantial ground for addressing the burgeoning challenge of smishing attacks.
    
\subsubsection{Hybrid approach}
Hybrid methods for smishing detection fully exploit the strengths offered by both conventional machine-learning and deep-learning mechanisms, thereby augmenting accuracy and reducing the possibility of false positives. A hybrid algorithm comprising CNN and LSTM gives an accuracy score of 99.74\%, which efficiently identifies significant features from text messages \citep{mehmood2024enhancing}. In addition, deep learning models tend to obtain higher accuracies than traditional algorithms as they automatically learn relevant features, resulting in fewer accuracies where real messages are misclassified as malicious. Another hybrid method \citep{jaafar2023iot} integrates predictive contextual embeddings with various machine learning techniques for smishing. Overall, models of this kind would appear to have some potential to reinforce cybersecurity against smishing threats, undoubtedly improving user protection. 

\subsubsection{Explainability and transparency of detection models}
In the area of smishing detection, machine learning models have become powerful tools. However, a critical aspect often overlooked is understanding how these models reach their conclusions. This section dives into Model Explainability, a rapidly growing field that aims to shed light on the decision-making processes within machine learning models. By employing techniques like SHAP (SHapley Additive exPlanations) or LIME (Local Interpretable Model-agnostic Explanations), we can gain valuable insights into the features and patterns that most influence the model's classification of a message as smishing or legitimate. This understanding not only fosters trust in the model's performance but also helps us identify potential biases or limitations that might require further refinement.

      %  \begin{itemize}
            
        
       % \end{itemize}

%-------- Comparison table 2 ----------------------%
\begin{table*}[!t]
\caption{Critical Analysis of Smishing Defense Measures Related Literature}
\label{tab:review-2}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|}
\hline
%\textbf{Sl.} & 
\textbf{Reference} & \textbf{Countermeasure Approach Category} & \textbf{Strengths} & \textbf{Weaknesses} \\
%& \textbf{Reference} \\ 

\hline

\multicolumn{1}{|p{8em}|}{NAHAPETYAN et al., 2024\citep{on_phishing_tactics_nahapetyan2023sms}} &
\multicolumn{1}{p{17em}|}{Analyzed 200 million+ messages, found thousands of \textbf{phishing campaigns}. Phishers use cloud infrastructure.} & 
\multicolumn{1}{p{17em}|}{Decades of anti-phishing expertise used, but tools have limitations.}& 
\multicolumn{1}{p{17em}|}{Used common tools (e.g., VirusTotal) but may miss some scams (data source bias).}\\ 

\hline

\multicolumn{1}{|p{8em}|}{TIMKO et al., 2023\citep{commerial_anti_smishing_timko_2023}} &
\multicolumn{1}{p{17em}|}{Compared message delivery across services, studied scam tactics \& link types.} & 
\multicolumn{1}{p{17em}|}{Use recent smishing messages for testing and novel approaches for collecting smishing data sets} & 
\multicolumn{1}{p{17em}|}{Few public datasets for testing scams; removed personal info from data.} \\
%\multicolumn{1}{p{4em}|}{TIMKO et al, 2023 \citep{commerial_anti_smishing_timko}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{24} &    
\multicolumn{1}{|p{8em}|}{KANAOKA et al., 2023\citep{kanaoka2023beyond}} &
\multicolumn{1}{p{17em}|}{Mobile smishing tackles limitations with image analysis, prototyping an \textbf{Augmented Reality} defense system. } & 
\multicolumn{1}{p{17em}|}{Offers a broader detection range with explores image analysis.} & 
\multicolumn{1}{p{17em}|}{Requires an additional device (AR glasses) for full functionality, impacting accessibility.} \\
%& \multicolumn{1}{p{4em}|}{Kanaoka et al., 2023 \citep{kanaoka2023beyond}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{23} &    
\multicolumn{1}{|p{8em}|}{NJUGUNA et al., 2021\citep{njuguna2021model}} &
\multicolumn{1}{p{17em}|}{Smishing defense system identifies \& alerts users, authenticates senders, and filters content using Naive Bayes.} & 
\multicolumn{1}{p{17em}|}{Focuses on \textbf{user awareness}, combines sender authentication, content filtering, and user notification.} & 
\multicolumn{1}{p{17em}|}{Relies on a Naive Bayes classifier and lacks details about evaluation methods.} \\
%& \multicolumn{1}{p{4em}|}{Njuguna et al., 2021 \citep{njuguna2021model}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{17} &    
\multicolumn{1}{|p{8em}|}{AKANDE et al., 2023\citep{smsprotect_akande}} &
\multicolumn{1}{p{17em}|}{\textbf{Mobile app} for spam SMS uses rules-based ML, not smishing prevention. User decides what to keep.} & 
\multicolumn{1}{p{17em}|}{Accuracy 98.08\%, used C4.5 algorithm to handle missing data and RIPPER algorithm outperformed C4.5 PART for accuracy.} & 
\multicolumn{1}{p{17em}|}{SMS spam detection struggles with missing data and limited features (C4.5 algorithm).} \\
%& \multicolumn{1}{p{4em}|}{Akande et al, 2023 \citep{smsprotect_akande}}\\

\hline


%\multicolumn{1}{|p{0.4em}}{16} &    
\multicolumn{1}{|p{8em}|}{KANAOKA et al., 2023\citep{kanaoka2023beyond}} &
\multicolumn{1}{p{17em}|}{\textbf{Cross-device approach}, using augmented reality (AR) glasses and URL analysis} & 
\multicolumn{1}{p{17em}|}{Cross-device detection, reduced device vulnerability, and user engagement} & 
\multicolumn{1}{p{17em}|}{Dependence on AR technology, camera limitations, and user acceptance.} \\ 
%& \multicolumn{1}{p{4em}|}{BOUKARI et al, 2021 \citep{mldetect_smishing_frauds_boukari}}\\

\hline

%\multicolumn{1}{|p{0.4em}}{16} &    
\multicolumn{1}{|p{8em}|}{BLANCAFLOR et al., 2021\citep{blancaflor2021let}} &
\multicolumn{1}{p{17em}|}{Emphasizes that trust and curiosity drive phishing link interaction, regardless of device security.} & 
\multicolumn{1}{p{17em}|}{Comprehensive platform comparison, \textbf{user behavior analysis, and realistic campaign} execution.} & 
\multicolumn{1}{p{17em}|}{Limited sample size, static security assessment, and single campaign design.} \\ 
%& \multicolumn{1}{p{4em}|}{BOUKARI et al, 2021 \citep{mldetect_smishing_frauds_boukari}}\\

\hline

\multicolumn{1}{|p{8em}|}{MISHRA et al., 2019
\citep{mishra2019sms}} &
\multicolumn{1}{p{17em}|}{Provided a comprehensive resource for users and researchers on identifying and countering smishing attacks.} & 
\multicolumn{1}{p{17em}|}{Comprehensive overview, practical recommendations, and insightful literature review.} & 
\multicolumn{1}{p{17em}|}{Focus on user awareness, limited discussion on technological solutions, and lack of experimental validation.} \\
%& \multicolumn{1}{p{4em}|}{KARHANI et al, 2023 \citep{karhani_phishing_2023}}\\

\hline

\multicolumn{1}{|p{8em}|}{SIADATI et al., 2017
\citep{siadati2017mind}} &
\multicolumn{1}{p{17em}|}{By preventing social engineering attacks that steal authentication codes, this work improves \textbf{SMS-based 2FA security}.} & 
\multicolumn{1}{p{17em}|}{Targeted solution for 2FA security, effective experimental approach, and scalable and lightweight tools.} & 
\multicolumn{1}{p{17em}|}{Focus on SMS-based 2FA only, limited social engineering scenarios, potential user adaptation required.} \\
%& \multicolumn{1}{p{4em}|}{KARHANI et al, 2023 \citep{karhani_phishing_2023}}\\

\hline

\multicolumn{1}{|p{8em}|}{SHAHRIAR et al., 2015
\citep{shahriar2015mobile}} &
\multicolumn{1}{p{17em}|}{Addresses mobile phishing attacks that exploit mobile devices' popularity and \textbf{user behavior}.} &
\multicolumn{1}{p{17em}|}{Awareness building, broad coverage of phishing types, and practical recommendations.} & 
\multicolumn{1}{p{17em}|}{Limited focus on technological solutions, device and OS variability.} \\
%& \multicolumn{1}{p{4em}|}{KARHANI et al, 2023 \citep{karhani_phishing_2023}}\\

\hline

\end{tabular}
}
\end{table*}

\subsection{Anti-Smishing Tools and Defense Countermeasures}
    \subsubsection{Anti-smish tools as defense} \citep{commerial_anti_smishing_timko_2023}
    \subsubsection{Mobile-based solutions and user alerts as defense}
     Secure Mobile Technologies: Explores the use of security features on mobile devices, such as SMS filtering and two-factor authentication, to prevent smishing attacks from succeeding \citep{a_study_psy_siddiqi}. Mobile applications offer a promising approach to smashing detection by analyzing incoming text messages for suspicious content, links, and sender information. These apps can leverage machine learning algorithms to identify red flags based on known smishing tactics and real-time threat intelligence. Mobile app integration with SMS filtering services can automatically block potential smishing messages before they reach the user. However, the effectiveness of mobile app-based solutions depends on user adoption and the ability to keep detection models updated against evolving smishing techniques. Balancing user privacy with robust detection capabilities remains a key challenge for this approach. {\color{red}need to cite these 2 papers here \citep{siadati2017mind} \citep{wang2024verisms}}



    \subsubsection{User training and awareness practices as defense}
    {\color{red}User Awareness and Education: Emphasizes the importance of educating users to recognize red flags and develop safe practices for interacting with SMS messages \citep{blancaflor2021let}. Highlights the importance of training users to identify smishing attempts through simulations and education on safe browsing habits \citep{clasen2021friend}.} User awareness training plays a vital role in empowering individuals to identify and avoid smishing attempts. Training programs can educate users about common smishing tactics, suspicious message elements, and best practices for responding to text messages. Interactive simulations and real-world scenarios can enhance user engagement and retention of key defensive strategies. Effective user awareness training should be ongoing and cater to diverse learning styles to ensure widespread adoption and positive behavioral change. User awareness training, combined with technological solutions, can create a multi-layered defense against smishing attacks.


\subsubsection{Law enforcement and regulatory efforts as defense}
Law Enforcement and Regulatory Efforts: Discusses the role of law enforcement in tracking cybercriminals and the development of regulations to protect consumers from smishing threats \citep{faklaris2024mitigating}.
        

\subsection{Generating and Publishing SMS and Spam Message Datasets}
\subsubsection{Available SMS datasets}
We have observed six publicly available datasets so far listed in table \ref{table:sms_data_details} related to smishing which are Enron Email Spam \citep{enron_vangelis2006spam}, British English SMS \citep{british_sms_dataset2011}, UCI Machine Learning Repository SMS Collection \citep{UCI_sms_dataset}, The National University of Singapore (NUS) SMS Corpus \citep{nus_chen2013creating}, SMS Gateways dataset \citep{on_phishing_tactics_nahapetyan2023sms} and the Smishtank dataset \citep{timko2024smishing}. Although the Enron dataset is curated from spam emails, it has been applied to detect SMS phishing as the textual contents share characteristics similar to phishing messages. Also, only two of the datasets, SMS Gateways and the Smishtank, are the most recent being published after 2023, while all the other datasets were published almost a decade before that. The datasets are provided in text, CSV, docs and JSON format and three of the datasets, Enrorn, English SMS, and the UCI ML Repo are labeled with {\tt Ham} and {\tt Spam} categories. Interestingly, all the message samples in the Smishtank and the SMS Gateways datasets consist of the smishing messages because the Smishtank dataset is curated from user input of the instance record of smishing messages and maintained by a research team and the author of the SMS Gateways dataset collected over 200 million SMS messages from 11 public SMS gateways on the web and later confirmed the URL within the messages as phishing resulting a dataset of 68029 smishing messages (table \ref{table:sms_data_details}). 

\subsubsection{Basic analysis of available datasets}

Among the three datasets, Enron, NUS Corpus, and the SMS Gateways dataset contain a higher number of message entries compared with other datasets with the count of 33,715, 55,835, and 68,029 instances respectively. Table \ref{table:sms_data_details} also provides basic statistics on the six publicly available datasets. The average length of the messages in the Enoron dataset is higher than the other datasets as this dataset contains email spam messages. From the other 5 smishing datasets, in Smishtank, the average message length is 176.96 which is the highest among this group. The messages in NUS Corpus seem to be the smallest in size as the average length is only 52.01 characters. Surprisingly, in the two labeled datasets, English SMS and UCI ML Repo, the average length of the {\tt Ham} messages are quite identical with average characters of 78.89 and 71.47. The same goes for the {\tt Spam} messages for both of these datasets with an average character length of 136.4 and 138.68 respectively. We have also provided the information for each dataset on the count and percentage of messages that contain URL, phone number, and email within them. Obviously, the Smishtank (85.98\%) and the SMS Gateways dataset (99.14\%) contain a higher number of messages that have URLs in them because these datasets contain only the smishing instances. Enron dataset also contains a significant number of messages (19.17\%) that have URLs in them. For the English SMS dataset, we have observed a notable amount of messages (20.11\%) with phone numbers embedded inside the messages. However, we have seen fewer messages that have email addresses embedded with the messages for every highlighted dataset on table \ref{table:sms_data_details}.

\begin{table*}[!t]
    \centering
    \caption{Summary of Publicly Available SMS Datasets}
    \vspace{-0.4em}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lll|*{9}{l}|rrr}
        \midrule
        \multirow{2}{*}{Dataset (year)} & \multirow{2}{*}{Format} & \multirow{2}{*}{Labeled} & \multicolumn{3}{c}{\# Instances} & \multicolumn{3}{c}{Avg. $\left| message \right|$} & \multicolumn{3}{c|}{Std. $\left| message \right|$}  & \multirow{2}{*}{\#URL Message} & \multirow{2}{*}{\#Phn Message} & \multirow{2}{*}{\#Email Message}\\
        
        \cline{4-12}
         & & & full & ham & spam & full & ham & spam & full & ham & spam\\
        \midrule

         Enron Email spam (2006) \citep{enron_vangelis2006spam} & .txt & yes & 33715 & 16545 & 17170 & 1446.84 & 1651.67 & 1249.47 & 4245.90 & 5758.30 & 1923.70 & 6463 (19.17\%)& 2707 (8.03\%) & 62 (0.18\%)\\

         
        English SMS (2011) \citep{british_sms_dataset2011}  & .doc & yes & 875 & 450 & 425 & 106.82 & 78.89 & 136.4 & 46.78 & 42.34 & 30.13 & 99 (11.31\%)& 176 (20.11\%) & 9 (1.03\%)\\

        UCI ML Repo (2011) \citep{UCI_sms_dataset} & .txt & yes & 5574 & 4827 & 747 & 80.48 & 71.47 & 138.68 & 59.84 & 58.32 & 28.85 & 495 (8.88\%)& 336 (6.03\%) & 16 (0.29\%)\\

        NUS Corpus (2015) \citep{nus_chen2013creating} & .json & no & 55835 & - & - & 52.01 & - & - & 54.17 & - & - & 3433 (6.15\%)& 52 (0.09\%) & 28 (0.05\%)\\


        SMS Gateways (2023) \citep{on_phishing_tactics_nahapetyan2023sms} & .csv & no & 68029 & - & - & 112.45 & - & - & 31.89 & - & - & 67442 (99.14\%)& 54 (0.8\%) & 807 (1.19\%)\\
        
        Smishtank (2024) \citep{timko2024smishing} & .csv & no & 1091 & - & - & 176.96 & - & - & 121.28 & - & - & 938 (85.98\%)& 38 (3.48\%) & 6 (0.55\%)\\

        
        \hline
    \end{tabular}
    \label{table:sms_data_details}
  }
\end{table*}

\ignore{
\begin{table*}[!t]
    \centering
    \caption{Summary of Publicly Available SMS Phishing Related Datasets}
    \resizebox{0.999\textwidth}{!}{
    \begin{tabular}{rrr|*{9}{c}|lll}
        \hline
        \multirow{2}{*}{Dataset} & \multirow{2}{*}{Format} & \multirow{2}{*}{Labeled} & \multicolumn{3}{c}{\# Instances} & \multicolumn{3}{c}{Avg. $\left| message \right|$} & \multicolumn{3}{c|}{Std. $\left| message \right|$}  & \multirow{2}{*}{\#URL Message} & \multirow{2}{*}{\#Phn Message} & \multirow{2}{*}{\#Email Message}\\
        \cline{4-12}
         & & & full & ham & spam & full & ham & spam & full & ham & spam\\
        \hline

        ENRON Email spam(2006) \citep{enron_vangelis2006spam} & .txt & yes & 33715 & 16545 & 17170 & 106.82 & 78.89 & 136.4 & 46.78 & 42.34 & 30.13 & 99 (11.31\%)& 176 (20.11\%) & 9 (1.03\%)\\

        
        British & .doc & yes & 875 & 875 & 875 & 106.82 & 78.89 & 136.4 & 46.78 & 42.34 & 30.13 & 99 (11.31\%)& 176 (20.11\%) & 9 (1.03\%)\\

        NUS & .json & no & 55835 & - & - & 52.01 & - & - & 54.17 & - & - & 3433 (6.15\%)& 52 (0.09\%) & 28 (0.05\%)\\

        UCI & .txt & yes & 5574 & 5574 & 5574 & 80.48 & 71.47 & 138.68 & 59.84 & 58.32 & 28.85 & 495 (8.88\%)& 336 (6.03\%) & 16 (0.29\%)\\

        Smishtank & .csv & no & 1091 & - & - & 176.96 & - & - & 121.28 & - & - & 938 (85.98\%)& 38 (3.48\%) & 6 (0.55\%)\\
        \hline
    \end{tabular}
    \label{table:dat_details}
    }
\end{table*}
}

\begin{table*}[!h]
\centering
\caption{Analysis of Existing Models and Their Performance Evaluations Using Both Public and Private Datasets}
\label{tab:dataset_result_sum}
\resizebox{0.95\textwidth}{!}{
\begin{tabular}{c|c|c|c|cc}
\toprule
        Data Availability  &     Reference &                                      Datasets Used &                               Best Algorithm Model & Accuracy &  F1 Score \\
\midrule

  %2 &   ALKHALIL et al, 2021 \citep{phishing_comp_study_alkhalil} &                                                - &                                                - &      - &       - \\
     & BOUKARI et al. 2021 \citep{mldetect_smishing_frauds_boukari}& Private &    RF  &      0.9815 &       0.9257 \\


    Private  &   NJUGUNA et al. 2021 \citep{njuguna2021model} & Private & NB & 0.9375 & 0.9333 \\

      &    SEO et al., 2024 \citep{seo2024device} &  Private (KISA) & Char-CNN & 0.9960 & 0.9944 \\


  \midrule


        &   GHOURABI et al. 2020 \citep{ghourabi2020hybrid} & UCI ML Repo + Private (Arabic) & CNN-LSTM & 0.9837 & 0.9148 \\
  
  % This is a phishing paper
  \ignore{
  4. &   &    EJAZ et al. 2023 \citep{life_long_phsising_ejaz}&                                           Private &                      Continual Learning (LWF, EWC) &  94 (TP) &       - \\}


  
    & GHOURABI et al. 2021 \citep{smdetector_ghourabi}&                                            UCI ML 
  Repo + Private (Arabic) &                                            BERT-FC &   0.9963 &    0.9558 \\

  
       &  JAIN et al. 2022 \citep{content_url_analysis_jain}& UCI ML 
  Repo + Private (URL Phishing) &                                     Voting (RF, KNN, ETC) &   0.9903 &       - \\

  

  
   Public + Private &   MISHRA et al. 2022 \citep{smishing_detector_security_model_mishra_2020}& UCI ML Repo + Private (Pinterest Image)  &                                       NB  &   0.9629 &       0.9200 \\

  
    &  MISHRA et al. 2022 \citep{implement_smishing_detector_mishra_2022}& UCI ML Repo + Private (Pinterest Image) &   ANN &    0.9740 &    0.8672 \\

 
   &   MISHRA et al. 2023 \citep{dsmish_mishra_2023}&                                 UCI ML Repo + Private (Pinterest Image) &             MLP Back Propagation &   0.9793 &       0.8150 \\


     &  KARHANI et al. 2023 \citep{karhani_phishing_2023}& NUS Corpus + Private (TELUS) & RF + SVC &    0.9940  &    0.9901 \\

  
 %12 &    NEUPANE et al, 2015 \citep{multi_modal_neupane}&                                                - &                                                - &      - &       - \\
 %11. &     RAHMAN et al, 2022 \citep{user_really_respond_rahman}&                                                - &                                                - &      - &       - \\
 %11. &         SIDDIQI et al. \citep{a_study_psy_siddiqi}& Ebbu2017. Secondary online sources  &                                                - &      - &       - \\
% 11. &      TIMKO et al, 2023 \citep{commerial_anti_smishing_timko}& UCI machine learning SMS spam collection and Private &                                                - &      - &       - \\
 %16 & NAHAPETYAN et al, 2023 \citep{on_phishing_tactics_nahapetyan2023sms}&                                            Private &                                                - &      - &       - \\
 


 \midrule





 
      &   MISHRA et al. 2019 \citep{mishra2019content} & UCI ML Repo & OneVsRestClassifier & - & - \\



   &  SONOWAL, 2020 \citep{sonowal2020detecting} & UCI ML Repo & AdaBoost & 0.9867 & 0.9486 \\


 
  Public  &   ULFATH et al. 2022 \citep{ulfath2022detecting} & UCI ML Repo & SVM & 0.9839 & 0.9637 \\

 

       &  HOSSAIN et al. 2022 \citep{spam_filtering_cnn_lstm_hossain}&        UCI ML 
  Repo  &                                           CNN-LSTM &    0.9840 &    0.9800 \\
 %15. & BLANCAFLOR et al. 2021 \citep{blancaflor2021let} & Private & - & - & - \\
 

  & SIDHPURA et al. 2023 \citep{sidhpura2023_fedspam:}& Enron + UCI ML Repo + English SMS &                                         DistilBERT &     0.9800 &       - \\



    & AKANDE et al. 2023 \citep{smsprotect_akande} &         UCI ML Repo  &                              PART (C4.5) &   0.9842 &       0.9840 \\
 
 %24 & KANAOKA et al., 2023 \citep{kanaoka2023beyond} & - & Google’s ML Kit API & 0.8519 & - \\
 
 %26 & CLASEN et al. 2021 \citep{clasen2021friend} & Private & - & - & - \\
 
 %28 & TIMKO et al. 2024 \citep{timko2024smishing} & Smishtank Dataset & - & - & - \\
 
\bottomrule
\end{tabular}}
\end{table*}

\subsubsection{Evaluation of current usages of these datasets}
In the previous studies related to smishing detection, there has been the implementation of private, public, and a mixture of both datasets as mentioned in table \ref{tab:dataset_result_sum}.  
Among the public datasets, the most frequent one is the UCI ML Repo dataset. The highest accuracy gained on this dataset is 0.9867 using the AdaBoost model. However, in terms of both accuracy and F-1 score, the most recent work of Akande {\textit{et al.}} \citep{smsprotect_akande} that leverage the PART (C4.5) model that has an accuracy of 0.9842 and F-1 score of 0.9840 should be considered as the highest performed one. Overall observation reveals that the researchers have utilized diverse sets of ML and DL models to make reliable smishing detection models. Although most of the works focus on the smishing with respect to the English language, there have been several few work that focuses on Arabic \citep{ghourabi2020hybrid, smdetector_ghourabi} and Korean \citep{seo2024device} language-based smishing detection. The private data is curated from various telecommunication companies and from individual trials as well as from user surveys and Pinterest images that are later converted into text messages manually.   

%-------- Comparison table 4 ----------------------%
\ignore{
\begin{table*}[!h]
\caption{Critical Analysis of Smishing Dataset Literature}
\label{tab:reveiw-4}
\resizebox{\textwidth}{!}{
\begin{tabular}{|l|l|l|l|}
\hline
%\textbf{Sl.} & 
\textbf{Reference} & \textbf{Key Attributes} & \textbf{Strengths} & \textbf{Weaknesses} \\
%& \textbf{Reference} \\ 

\hline


\multicolumn{1}{|p{4em}|}{%Phishing and Smishing Detection Using Machine Learning 
\citep{UCI_sms_dataset}} &
\multicolumn{1}{p{17em}|}{{\color{red}add details here.}} & 
\multicolumn{1}{p{17em}|}{{\color{red}add details here.}} & 
\multicolumn{1}{p{17em}|}{{\color{red}add details here.}} \\
%& \multicolumn{1}{p{4em}|}{KARHANI et al, 2023 \citep{karhani_phishing_2023}}\\

\hline


\end{tabular}
}
\end{table*}
}

%\footnote{here goes the published public datasets, and tables where various datasets are used in existing literature}


\subsection{Study to Understand User Perception and Psychology}

%-------- user-study driven literature table ----------------------%
\subsubsection{Users susceptibility to smishing attacks}
User behavior and perception are important in dealing with smishing attacks. As having a lack of knowledge in mobile security makes users easy targets for attackers \citep{mishra2019sms}, Illusion of knowledge is also dangerous in this field. The Term "security expertise bias" refers to a situation in which users with more security awareness are overly suspicious which decreases their ability to determine legitimate and phishing messages. This indicates that users with advanced security training are making mistakes when classifying benign messages and smishing. Users also showed vulnerability when they thought they were an account holder of an entity named in the message. In this case, they disregard fraudulent cues and fall into smishing. This suggests that having a sense of familiarity with security issues and the sender leads to the opposite result \citep{faklaris2023preliminary}. On the other hand, involvement with smishing is sometimes only for curiosity, even past experiences may not influence falling in it again, as the two-round setup of experiment in this study shows \citep{lutfor_23_codaspy_users_smished}. Users’ routines also influence them in smishing susceptibility. Research shows that frequent use of social media or banking apps makes messages in those contexts more trustworthy. For example, users with more spending time on social media, are more vulnerable to social media-related messages \citep{kumarasinghe2023user}. Finally, based on a habit, Users often enter credentials or respond to prompts without careful consideration \citep{mishra2019sms}.
%\noindent (i)	Demographic Factors Impacting Susceptibility 



%\footnote{here we create table for user study and have column presenting participant size, study type, ethnic diversity, age group diversity, racion or other forms of diversity to understand the gaps from existing literature}
\subsubsection{Visual ques for detecting smishing}


Visual Cues are kind of elements designed by Attackers particularly to intimidate or lure users to benefit from their emotions \citep{lutfor_23_codaspy_users_smished}. users also can determine whether a message is phishing or legitimate using these cues. The visual Cues help users to detect suspicious patterns which are commonly Integrated into phishing attempts \citep{clasen2021friend}. We have reviewed these visual cues and divided them into four main categories. In what follows, we discuss some of those important visual cues:

\noindent \textbf{(i) Meta-Data based cues:}

\textbf{i-A) Fake URLs:} indicates Fraud. These URLs often do not match other message attributes. Users who usually focus on these URLs are more likely to detect phishing messages \citep{timko2023quantitative}. Research particularly found that a mismatch between URL and claimed service is frequent \citep{clasen2021friend}.

\textbf{i-B) Shortened URLs:} Using a shortened URL in a message is a common strategy in smishing. This Cue is widely Identified as Suspicious and helps to detect phishing messages \citep{clasen2021friend}.

\textbf{i-C) Suspicious URLs:} Attackers may use a shortened or deformed shape that looks similar to the original URL but they modified it partially to Trick users into clicking on it \citep{dsmish_mishra_2023}. These URLs often redirect users to a phishing website that also looks similar to a legitimate website and motivate them to enter their personal data for example login information or credit card numbers. Another form of suspicious URL which is known as Self-Answering Links (SAL), pretends as a subscribe-unsubscribe link for a service but includes a link to a malicious website \citep{mishra2019content}.

\textbf{i-D) Spoofed Area Code:} In this process, attackers used local area codes that are familiar to users so that user. These messages appear to have been sent from a close geographical location so users can trust more to them to respond \citep{lutfor_23_codaspy_users_smished}

\noindent \textbf{(ii) Content-based cues:}

\textbf{ii-A) Messages Containing Forms in Their URLs:}
Similar to Suspicious URLs, these messages contain URLs linked to a From, motivate users to enter their sensitive data such as login information or financial data \citep{mishra2019content}.

\textbf{ii-B) Messages Asking for Personal Information:}
These kinds of messages Ask their recipients to send back their sensitive data such as passwords or credit card credentials \citep{jain2019feature}. Attackers sometimes ask for this information indirectly; they first provide a phone number or email address and ask recipients to contact them. When they are contacted, attackers may ask them to send their personal and sensitive information for a fake reward like a coupon or gift \citep{mishra2019content}.

\textbf{ii-C) Messages Asking for an APK Download:}
These Smishing contain a link for downloading an APK file. Once downloaded, they are able to do different harmful activities on the destination device  \citep{mishra2019content}.

\textbf{ii-D) Call to Action (CTA):} Benign SMSs usually have a Transparent and Explicit Call to Action. In contrast, phishing messages ask recipients to act urgently \citep{timko2023quantitative}. However, using a call to action was discovered on some smishing campaigns. These messages encourage recipients to click on a suspicious link, contact the phone number mentioned in the message to have a conversation with attackers, or ask them to send back valuable information \citep{lutfor_23_codaspy_users_smished}.

\textbf{ii-E) Entity Identification:}
Entities also known as organization names or Brands, are a potential factor to identify smishing. Studies show that users are suspicious of entities. If the entity that sent the message is not well known, it could be considered phishing \citep{timko2023quantitative}. Attackers use this feature to lure users. They pretend as a known brand or organization like “Walmart” or a “Bank” to get the user’s trust. this sense of trust enables users to respond to these phishing messages respond \citep{lutfor_23_codaspy_users_smished}. 

{\color{red}3.2.6 \textbf{Scenario-Based Cues:}
The unusual context of messages (Scenario), especially if it does not match with the claimed sender, makes it a good candidate as a suspicious message \citep{timko2023quantitative}. Attackers use scenarios, too. They use Rewards or a sense of fear in their scenarios to trigger recipients to respond. Reward scenarios usually offer rewards, gifts, or job opportunities, while fear scenarios give a dangerous sense to users with tax-filling problems, or account login attempts. This fear feeling of losing personal data or legal punishment makes users engage with these messages \citep{lutfor_23_codaspy_users_smished}. }

\textbf{ii-F) Urgency Related Text Contents:}
Any kind of words or using specific linguistics that triggers a sense of urgency will make users act quickly. As we discussed before, those reward and fear-based scenarios have the most impact on users to give them a sense of urgency \citep{jain2019feature}.  

\noindent\textbf{(ii-G) Suspicious phase or keyword based cues:} Several studies used different methods like machine learning and text processing to find the most commonly used phrases or keywords in smishing attacks. The set of these phrases or words are as follows: \{`award', `congratulation', `winner', `alert', `claim', `activate', `verify', `attempts', `gift voucher', `blocked', `suspend', `unlock', `won', `prize', `subscribe', `activity', `update', `coupon', `refund', `call', `free', `text', `claim', `ur(your)', `like', `get', `cash', `you have been selected', `£'\} \citep{jain2019feature,content_url_analysis_jain,smdetector_ghourabi}.

\noindent \textbf{(ii-H) Poor grammar, misspelled words, and special characters based cues:}
Legitimate Messages usually use well-written structure and good grammar. In contrast, Phishing messages have a poor linguistic structure with grammatical and spelling problems \citep{clasen2021friend}. These Linguistic mistakes combined with replacing letters with symbols, special characters, and numerical values are sometimes used by attackers intentionally to bypass automatic spam detection systems and create ambiguous words to lure recipients \citep{dsmish_mishra_2023}. 




\subsubsection{Diversity of participants in existing smishing user studies}

In this section, we discuss and learn from various existing user study research, which are dedicated to understand users' interactions and perceptions when exposed to smishing, specially if demographic factors impact their susceptibility. 

\noindent \textbf{(i) Age-related Patterns:} While age does not always play a significant role in being susceptible to smishing \citep{yoro2023evidence}, some recent studies investigate younger adults (under 35) are more vulnerable to Smishing and older adults are doing better in identifying these types of messages \citep{faklaris2023preliminary}. Interestingly, research shows that people in the age range of 45-54 have the highest susceptibility (25\%), while the younger group had the lowest score (4.17\%) \citep{lutfor_23_codaspy_users_smished}. This low score which is coming from lower caution and financial experiments, is highly in contrast with their ability to categorize phishing messages, with rates exceeding 87\% \citep{clasen2021friend}.

\noindent \textbf{(ii) Gender Impacts:} Researchers showed an interest in considering Gender as one of the demographics in their susceptibility to smishing studies. Their findings have changed over time so that there is no significant difference in smishing vulnerability based on gender \citep{faklaris2023preliminary}. while both genders showed vulnerability to smishing attacks \citep{yoro2023evidence}. Prior findings reveal females had a slightly higher susceptibility (11.38\%) than males (9.86\%) \citep{lutfor_23_codaspy_users_smished}. Another study confirmed this idea where Females (68.5\%) were more susceptible to phishing attacks compared to Male (59\%) Participants \citep{yoro2023assessing}. In terms of categorizing legitimate and smishing messages, male participants had more accurate results (74.8\%) than female participants (71.9\%) \citep{clasen2021friend}.

\noindent \textbf{(iii) Impact of Educational Background:} Research shows that there is a direct correlation between Higher Education level and greater susceptibility in which people with a Doctoral degree had the highest susceptibility at 37.5\% and those with a high school degree or lower showed a susceptibility rate of 20\% and less. \citep{lutfor_23_codaspy_users_smished}. In addition, College students who are currently studying for a four-year degree were found to be highly susceptible \citep{faklaris2023preliminary}. It shows a descending distribution where First-year students were the most vulnerable (82.9\%) and it is decreasing during the next academic years in which Fourth-year and above students had the lowest rate (21.3\%) \citep{yoro2023assessing}.

%-----moe table 7----%




\begin{table*}[ht]
\centering
\caption{Critical Analysis of User-Study-Driven Smishing Research Studies}
\resizebox{\textwidth}{!}{
\begin{tabular}{p{0.5cm}|p{3.3cm}|p{0.75cm}|p{1.4cm}|p{3cm}|p{1.5cm}|p{2cm}|p{2cm}}
\hline
\textbf{Ref.} & \textbf{Key Idea} & \textbf{\# of Users} & \textbf{Study Type} & \textbf{Ethnic/Racial Diversity} & \textbf{Age Group Diversity} & \textbf{Education Level} & \textbf{Gender Diversity}\\
\hline

%\citep{a_study_psy_siddiqi} & &  & &  &  &  & - \\

%\hline

\citep{lutfor_23_codaspy_users_smished} & Analyzing message attributes and participant features to find why smishing works & 256 & Experimental & White, African American, Asian American, Mexican American, Native Hawaiian & 18-24 (4.17\% Fall Rate) to 45+ (25\% Fall Rate) & from less than high school to doctoral degree & - \\
\hline
\citep{clasen2021friend} & Investigate how participants classify Legitimate and smishing & 576 & Survey-based Quantitative & - & 18-21 (40.5\%), 22-25 (27.9\%), 26-30 (18\%), 31-40 (9.2\%), 41+ (4.4\%) & - & Male- 50\%, Female- 45\%, Other- 5\% \\
\hline
\citep{edwards2023smishing} & Studying user behavior and susceptibility to Smishing Attacks & 28 & Survey-based Behavioral & - & 18-21 & mostly had no technical skills & Males (32.1\%), Females (67.9\%)  \\
\hline
\citep{blancaflor2021let} & Evaluating users’ vulnerability to phishing attacks & 24 & Experimental & - & - & - & \\
\hline
\citep{yoro2023evidence} & Investigating how demographic factors impact vulnerability of undergraduate students & 480 & Quantitative Experimental & Nigerian university students & Under 21 (21.5\%), 21 to 25 (34.5\%), 26 and above (44.0\%) & 89.1\% domestic, 11.9\% International Undergraduate Students & Males (50.9\%), Females (49.1\%)  \\
\hline
\citep{bach2022targets} & Investigating the susceptibility to phishing attacks in participants from European countries with different educational levels & - & Quantitative analysis using fuzzy clustering & European countries & - & from low to medium and high educational background &  \\
\hline
\citep{faklaris2023preliminary} & Investigating demographic and contextual factors impacting the vulnerability to smishing attacks & 1007 & Survey-based demographic analysis & White/Caucasian (839), Black/African American (106) & 18-24 (232), 25-34 (70), 35-54 (312), 55-64 (173), 65+ (219) &  & Males (62\%), Females (36\%), Other (2\%) \\
\hline
\end{tabular}
}
\end{table*}





%\twocolumn[\columnbreak]


%---moe table 7 end --%




%\footnote{still need to address the rule-based column name to change to `detection method' and the row values can be rule-based, ml-based, dl-based, and others in Table 2}






%Smishing attacks pose a significant threat to mobile phone users, often leading to financial loss and identity theft.  To effectively combat this growing menace, researchers have explored various detection methods. This section critically reviews the existing research on smishing detection, synthesizes the key findings, and summarize them in several table to find the gaps in the current knowledge base. This study presents a comprehensive overview of the research landscape using a structured table. The table 1 categorizes detection methods into five key areas:

%\subsection{Detection Mechanisms}

% Akande et al. propose a mobile application, SMSPROTECT, to combat smishing attacks\citep{smsprotect_akande}. Recognizing the limitations of existing anti-spam solutions, SMSPROTECT combines a rule-based system with machine learning models (RIPPER and C4.5) to analyze incoming messages. The application classifies messages as spam or legitimate, but importantly, empowers users to make the final decision on keeping or discarding them. The authors highlight the user's role and evaluate the application's effectiveness using metrics like True Positive Rate and Precision. Overall, this research introduces a promising approach for user-centric smishing prevention on mobile devices. 

% In Another paper, Mishra et al. propose a system to detect smashing messages\citep{dsmish_mishra_2023}. Smishing is a fraudulent attack where attackers trick users into clicking on malicious links in text messages. The system uses two phases: Domain Checking Phase and SMS Classification Phase. The first phase checks the legitimacy of the URL in the message. The second phase analyzes the text content of the message and extracts features. The system uses a Backpropagation Algorithm to classify the message as spam or smishing. The authors claim their system achieves an accuracy of 97.93\%.


%\subsection{Defense Countermeasures}

%\subsubsection{User Study Based}

%\vspace{-0.9em}
%\subsubsection{Mobile Applications Based}


%\subsubsection{User Awareness Training}




%SMS content analysis-based work authored by Sandhya Mishra and Devpriya Soni \citep{smishing_detector_security_model_mishra_2020}, introduces an innovative system designed for the detection of smishing SMS attacks, a type of phishing that specifically targets smartphone users through text messages. The system employs a two-phase approach: the Domain Checking Phase and the SMS Classification Phase. It scrutinizes the authenticity of URLs in SMS messages, extracting five efficient features for machine learning classification. Impressively, the system achieves a high accuracy of 97.93\% in detecting smishing messages. The evaluation involves the use of SMS datasets, comparing the system with traditional classifiers, and utilizing a final dataset of 5858 text messages. Challenges addressed include the scarcity of real smishing datasets, analyzing abbreviated messages, and differentiating smishing from spam. The proposed system contributes to simplifying URL genuineness checks in SMS, and the case study on the Paytm smishing scam showcases its real-world applicability. The paper outlines future directions, suggesting the development of blacklists and the creation of signatures for search engine domain checks. The methodology involves the Backpropagation Algorithm and three traditional classifiers, utilizing features such as leet words and URL authenticity. The architecture of the backpropagation network, the overall working of the proposed model, and figures illustrating a Paytm scam message with leet words, prediction results of machine learning algorithms, and feature frequency are presented. The best-performing algorithm, the Backpropagation Algorithm, achieves an accuracy of 97.93\%. The paper offers a comprehensive exploration of a sophisticated system for smishing SMS detection and underscores its efficacy in addressing the inherent challenges of smishing attacks.

%Another research \citep{implement_smishing_detector_mishra_2022} by the same team introduced an innovative smishing detection system employing Artificial Neural Network (ANN). The paper aims to address the serious cybersecurity issue of smishing, where attackers target smartphone users through text messages. The proposed system extracts the best seven features of smishing SMS using Neural Network, with the URL feature demonstrating the highest effectiveness at 94\% accuracy. The Neural Network outperforms other classification algorithms, achieving an impressive accuracy rate of 97.40\%. The study focuses on authenticating URLs in SMS, leveraging real-time smishing messages collected from various sources, including the Almeida dataset and screenshots converted to text. The research employs a meticulous process, utilizing Neural Network as the ML model, identifying the seven most prominent features, and testing the selected feature set for accuracy. The study also proposes a comprehensive model for SMS and URL analysis, incorporating algorithms for URL inspection and keyword classification, determining the legitimacy of messages. Figures illustrate the iterative process of the ANN and the architecture of the 'Smishing Detector' model. Additionally, figure \ref{fig:smishing_detector_feature_wise_} shows which standalone feature works best for this system. The best-performing algorithm, Neural Network, attains an accuracy of 97.40\%, and the F1 Score is reported as 86.72 for Neural Network and 81.07 for Naive Bayes.

%The work \citep{life_long_phsising_ejaz} authored by Asif Ejaz et al. addresses the challenge of performance deterioration in traditional ML-based phishing detection models over time. They propose continual learning (CL) techniques, demonstrating a tolerable accuracy deterioration of 2.45\% compared to significant declines in other models. CL algorithms are positioned as a practical solution to maintain performance on evolving phishing attacks. The authors suggest further research on mitigating catastrophic forgetting and exploring adversarial training for CL-based models.

%In the paper \citep{mldetect_smishing_frauds_boukari} by Badr Boukari et al., the authors introduce a machine learning-based detection system for SMiShing frauds, aiming to protect victims from phishing and vishing frauds. The tool utilizes term frequency-inverse document frequency (TF-IDF) for assessing term importance and showcases performance through a demo. Naive Bayes achieves 86.17\% precision and 100\% recall, while Random Forest misclassifies some ham messages. The paper emphasizes the rise of telephony frauds, the complexity in detection, and the lack of a complete fraud detection system backed by AI. The machine learning-based tool presents a viable solution to protect victims and can be adapted for various fraud detection applications.

%The research \citep{smsprotect_akande} titled "SMSPROTECT: An automatic smishing detection mobile application" authored by Akandeet al., introduces an innovative mobile application designed to detect and prevent smishing attacks. Recognizing the widespread use of smartphones and the vulnerability of SMS as an attack vector, the paper aims to address the exploitation of SMS by hackers for smishing, a blend of SMS and phishing.

%The proposed solution employs a rule-based SMS service integrated with a machine learning model to analyze incoming SMS messages. Notably, the model, utilizing RIPPER and C4.5 classification algorithms, assesses the messages to distinguish between spam and legitimate ones. Unlike existing research that primarily focuses on detecting spam SMS, this paper emphasizes the prevention of smishing attacks. The user plays a pivotal role in the decision-making process, determining whether to retain or discard the messages based on the analysis results.

%The authors underscore the importance of user involvement in the decision-making process and highlight the performance evaluation of the rule-based SMS spam detection models. Evaluation metrics, including True Positive rate, False Positive rate, Precision, Recall, and F-Measure, were utilized to gauge the effectiveness of the developed mobile application. Simulated in real-time scenarios, the application intercepted incoming SMS, analyzed them, and classified them as spam or not spam.

%The research also emphasizes the significance of the proposed model's application, providing an overview of the methodology, including the rule-based technique for feature extraction, the use of clustering-based techniques, and the evaluation dataset derived from the UCL SMS spam dataset v.1. Overall, the paper contributes to the field by presenting an automatic smishing detection mobile application and demonstrating its efficacy in preventing smishing attacks.



%The very recent work on smishing by Aleksandr Nahapetyan \citep{on_phishing_tactics_nahapetyan2023sms} and their team goes into the intricate landscape of SMS phishing tactics and infrastructure, conducting an in-depth analysis that identifies over 600 distinct SMS phishing operations. With a 70\% increase in reported SMS and voice phishing attacks in 2022, the research extracts insights from over 200 million SMS messages, uncovering 67,991 phishing messages and 35,128 campaigns. Notably, SMS phishers leverage commodity cloud and web infrastructure, often reusing existing phishing kits from other modalities. The analysis reveals a trimodal distribution in the ratio of messages to destinations and emphasizes the urgency for robust defenses against SMS phishing. The paper suggests the active engagement of traditional SMS firewalls and A2P providers in URL crawling and incident response, backed by regulatory measures. Despite limitations, such as the challenging task of accurately detecting SMS phishing and the bias introduced by public SMS gateways, the paper provides valuable insights for cybersecurity professionals, policymakers, and researchers. The methods involve a comprehensive data collection process, including the aggregation of individual messages into campaigns and the identification of SMS phishing operations. While the dataset used is not explicitly mentioned, the paper utilizes various techniques, such as SpaCy's Named Entity Recognition and polyglot, for language identification and the analysis of three phishing kits. Key figures, including Figure \ref{fig:on_spam_3} and Figure \ref{fig:on_spam_9}, depict notable trends and phenomena observed during the research.

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{Figures/on_spam_3.png}
%   \caption{Figure indicating time campaign \citep{on_phishing_tactics_nahapetyan2023sms}}
%   \label{fig:on_spam_3}
% \end{figure}


% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{Figures/on_spam_9.png}
%   \caption{Bulk SMS services advertisement \citep{on_phishing_tactics_nahapetyan2023sms}}
%   \label{fig:on_spam_9}
% \end{figure}


%The research work \citep{commerial_anti_smishing_timko} conducts a comprehensive comparative study focusing on anti-smishing technology across bulk messaging services, carriers, and apps. With a focus on the rising threat of smishing attacks, the study aims to assess and improve the performance of commercial anti-smishing tools, offering valuable insights for the cybersecurity community, policymakers, and industry professionals. The analysis involves a standardized set of messages tested across various platforms within a 3-day period, evaluating the accuracy of smishing detection and filtering. Specific blocking tendencies and detection gaps in anti-smishing tools are identified, emphasizing the need for enhancement. The research contributes to smishing attack mitigation and advocates for the use of fresh and unvalidated smishing communications for testing, introducing smishtank.com as a publicly available source. The methods encompass a test bed development, validation of smishing messages by a security expert, and an analysis of the message blocking process in bulk messaging services, carriers, and third-party apps. The evaluation is based on the smish hit rate and benign strike rate, providing insights into tool performance shown in figure \ref{fig:commerce_tool}. Despite limitations, including the infeasibility of full permutations and the undisclosed techniques used by each tool, the study sheds light on critical areas for improvement. The dataset utilized comprises 50 ham SMS messages and 50 phishing messages from the UCI machine learning SMS spam collection, with data collected over two months and personally identifying information (PII) ethically removed. The study underscores the challenge of recognizing machine learning (ML) smishing detection approaches in commercial tools and concludes by emphasizing its contribution to industry understanding and addressing modern threats. 

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{Figures/commerce_tool.png}
%   \caption{Smishing vs Messenger, Carriers and Apps \citep{commerial_anti_smishing_timko}}
%   \label{fig:commerce_tool}
% \end{figure}

%Rahman et al. \citep{user_really_respond_rahman} investigated the effectiveness of smishing attacks on mobile users, revealing that 16.92\% of participants potentially fell for the smishing attack. The study explores user responses and demographic features, finding that a combination of user reply and click actions increases the odds of response. Notably, participants aged 18-24 had lower odds of responding to the scam, while African American and Mexican American participants had higher odds of falling for the scam. Users utilizing mobile devices for 11-20 hours a week also had higher odds of falling for the scam. The paper underscores smishing as a rising cybersecurity threat surpassing spam calls, emphasizing the need for greater user awareness and automatic detection mechanisms to combat smishing. The study identifies factors influencing the success rate of smishing scams, including user demographics, and advocates for carrier intervention to block smishing messages. Ethical considerations regarding the collection of participants' personal information are addressed, with the paper following standard Institutional Review Board (IRB) protocols to mitigate risks. Smishing experiments were conducted to measure efficacy, factors influencing success rates were identified, and the study emphasizes the need for user awareness and automatic detection mechanisms. 

%The research paper \citep{phishing_comp_study_alkhalil} authored by Zainab Alkhalil et al., addresses the pervasive issue of phishing attacks, a prominent form of cybercrime targeting personal information. The authors assert that existing countermeasures fall short in effectively combating sophisticated phishing attacks, prompting the need for a more nuanced understanding of the attack lifecycle. To this end, the paper introduces a new anatomy of phishing, offering a detailed examination of attack phases, attacker types, vulnerabilities, threats, targets, attack mediums, and techniques. This comprehensive approach aims to provide multifaceted countermeasures that not only consider technical aspects but also address human vulnerabilities. The paper underlines the evolving nature of phishing attacks, extending beyond traditional email-based schemes to encompass new mediums such as social media, voice, and SMS. The proposed anatomy serves as a framework to enhance awareness and understanding of various facets of phishing attacks. Furthermore, the authors emphasize the importance of tailored laws and legislations specifically addressing phishing, as current legal frameworks may be insufficient. The paper calls for a holistic approach to mitigate phishing threats, including evaluating existing countermeasures, proposing new preventive strategies, and fostering awareness regarding the diverse tactics employed by attackers. Overall, the research contributes to the ongoing efforts to combat cyber threats by shedding light on the intricacies of phishing attacks and advocating for a comprehensive defense strategy.

%\subsubsection{Psychological Study}

%The research work \citep{a_study_psy_siddiqi} discusses engineering-based cyberattacks, which exploit human vulnerabilities for malicious purposes. The paper emphasizes the difficulty in countering these attacks due to their high effectiveness and obscurity. It provides an in-depth analysis of social engineering attack tactics, highlighting the need for a comprehensive understanding to develop effective countermeasures. The study discusses existing approaches, including machine learning-based methods, aimed at thwarting social engineering attacks. It underscores the importance of recognizing linguistic and psychological factors in machine learning-based approaches, exploring vulnerabilities, and understanding human behavior in the context of social engineering attacks. The paper further addresses recent and prominent social engineering attacks, the significance of security awareness, and the necessity of a cybersecurity approach involving human factors. It proposes a systematic knowledge framework for analyzing and mitigating social engineering attacks, with future work focused on designing a systematic flow to handle such cyber threats. The study utilizes the Ebbu2017 dataset for model training and incorporates a secondary dataset from various internet resources, although the specific link is not provided. The paper introduces machine learning models, including deep learning methods, for pattern recognition in emails, SMS, malicious links, and calls, utilizing natural language processing (NLP). It explores linguistic features of social engineering for higher detection rates and integrates cognitive and psychological factors into machine learning-based approaches. Additionally, the paper discusses the use of deepfake techniques, generated through generative adversarial networks (GANs), in social engineering attacks, highlighting concerns about handling misinformation in deep learning-based approaches for SMS and URL analysis.


%Though this research work \citep{multi_modal_neupane} is done a while ago they shows the realm of cybersecurity, specifically focusing on phishing detection and malware warnings through neurophysiological measures. The study utilizes Electroencephalogram (EEG) cognitive metrics and eye gaze patterns for analysis, revealing that users spend more time analyzing malware warnings than phishing indicators. Users' attention control is identified as a crucial factor influencing accuracy in phishing detection, and their susceptibility to phishing attacks is linked to personality traits. Participants show higher engagement and task performance when processing warnings, with attention control training identified as a potential avenue for improving phishing detection accuracy. Real-time neural and eye gaze features are proposed as indicators of users' "alertness" state, emphasizing the need for future research to design and validate automated mechanisms. The paper combines EEG cognitive metrics and eye gaze patterns in a multi-modal neuro-physiological approach, offering insights into users' cognitive responses to security tasks. It underscores the challenges users face in identifying phishing websites, as they fail to do so more than 37\% of the time. However, users generally heed warnings about 85\% of the time. The study's methodology, encompassing statistical tests, realistic set-ups, and neuro-physiological measures, contributes to the understanding of user-centered security in cybersecurity. The paper acknowledges limitations, such as the study's lab setting possibly not reflecting real security risks, and proposes future research directions to enhance the credibility of human decisions in user-centered security systems. The authors present a comprehensive exploration of the intricate interplay between neural responses, eye focus, and task performance in the context of phishing detection and malware warnings, offering a foundation for further advancements in user-centered cybersecurity.

%\subsection{Messasge Analysis}
%\subsubsection{URL Analysis}
%Mishra and Soni \citep{smishing_detector_security_model_mishra_2020} introduce the "Smishing Detector," a robust security model designed to counter text message-based phishing attacks. Comprising four modules—SMS Content Analyzer, URL Filter, Source Code Analyzer, and APK Download Detector—the model demonstrates a superior overall accuracy of 96.29\%. Notably, the Naive Bayes classifier excels in keyword classification within the SMS Content Analyzer. The prototype, developed using the tkinter package, effectively reduces false-positive results in smishing detection. Addressing gaps in current smishing detection models, the research emphasizes the escalating threat landscape and the need for comprehensive security coverage. The Smishing Detector surpasses existing models by covering a wider range of security aspects. The paper highlights the limitations of current methodologies and contributes practical implications for enhancing smishing attack security. Methodologically, the paper details the use of the Naive Bayes Classification Algorithm, URL inspection, source code analysis, and APK Download Detector. Although a dataset is referenced, a direct link is not provided. The best-performing algorithm, Naive Bayes, achieves 96.29\% accuracy, with F1 Score information not provided. Overall, the paper presents a concise and insightful exploration of the Smishing Detector, its validation, and contributions to smishing attack detection.


%The paper \citep{smdetector_ghourabi} introduces "SM-Detector," a hybrid security model designed to detect smishing messages in mobile environments. This innovative model combines three detection methods for enhanced efficiency: identification of malicious URLs, analysis of suspected words, phone numbers, and emails using regular expression analysis, and classification of messages through BERT-based algorithms. The "SM-Detector" includes a user-friendly mobile application for SMS checking and reporting smishing messages, accommodating mixed-text messages in both Arabic and English. The experimental evaluation showcases an exceptional accuracy rate of 99.63\%.

%The proposed model is particularly noteworthy for its ability to seamlessly handle diverse text messages, its inclusion of a user-friendly mobile application, and the impressive experimental accuracy. The combination of heuristic methods and the application of pretrained BERT models for classification sets "SM-Detector" apart as an efficient system for detecting smishing messages. The paper sheds light on the challenges of smishing detection, offering a comprehensive solution that leverages advanced techniques.

%The hybrid model's success lies in its three-pronged approach: identification of malicious URLs, analysis of suspected words, and classification through BERT-based algorithms. The experimental evaluation, although lacking specific information on the dataset used, underscores the effectiveness of "SM-Detector," boasting a remarkable accuracy of 99.63\%. Figure \ref{fig:sm-detector} shows the architecture of the BERT-based classifier, providing visual insights into the model's operation. The best-performing algorithm, BERT-FC, attains a superior accuracy rate of 99.63\%, as reflected in the reported F1 Score of 0.955831.

% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=\linewidth]{Figures/sm-detector.png}
%   \caption{SM-detector architecture \citep{smdetector_ghourabi}}
%   \label{fig:sm-detector}
% \end{figure*}

%In the study \citep{content_url_analysis_jain}  the authors, Ankit Jain et al, present a comprehensive and efficient strategy for detecting smishing SMS, a fusion of SMS and phishing attacks. The proposed approach integrates content and URL analyses to enhance detection accuracy. Notably, the authors employ a TF-IDF weighting framework to identify rare words within SMS messages and utilize a synthetic minority oversampling technique to balance the training dataset, ensuring a more robust model. The model encompasses both a URL phishing classifier and a text classifier, synergizing logistic regression, KNN, RF, and ETC for optimal performance. Remarkably, the proposed approach achieves outstanding results, boasting a 99.03\% accuracy and an impressive 98.94\% precision rate. The authors recognize the limitations of existing anti-smishing solutions and advocate for a more holistic approach. They suggest future work involving the integration of third-party applications for URL classification, potentially improving the system's efficiency and speed. Moreover, the proposal includes the development of a dedicated mobile application to alert users about incoming smishing messages, thereby contributing to real-time threat detection and user awareness. The study emphasizes the rising threat of smishing attacks, especially during the Covid-19 pandemic, and underscores the need for advanced tools that can effectively detect such attacks from multiple angles. By combining both SMS content and URL analyses, the proposed method offers a nuanced and sophisticated solution. The authors utilize logistic regression, KNN, RF, and ETC classifiers in a voting ensemble to achieve superior accuracy. Figures within the paper visually represent the steps involved in preprocessing smishing messages, word clouds for smishing messages and phishing URLs, and the accuracy and precision of various models shown in figure \ref{fig:content_url_analysis} used for building the URL phishing classifier.

% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{Figures/content_url_analysis.jpg}
%   \caption{Accuracy and Precision of oversampled TF‐IDF vectorized data set \citep{content_url_analysis_jain}}
%   \label{fig:content_url_analysis}
% \end{figure}


%\subsection{Model Explainability}



%The only research work which has tried explaining their model is "FedSpam," by Sidhpura et al \citep{sidhpura2023_fedspam:}, a pioneering privacy-preserving SMS spam prediction system employing a federated learning approach. The proposed model, leveraging DistilBERT, is trained on mobile clients' SMS data, with local model weights sent to a central server for aggregation. The iterative process enhances the model's resilience to evolving spam techniques, achieving an impressive 98\% accuracy on the validation set. The paper underscores the vulnerability of SMS to spam exploitation, emphasizing the adoption of federated learning for on-device spam classification. Notably, the DistilBERT model preserves SMS data privacy by aggregating weights on the server. The literature survey provides a comprehensive overview of related work, positioning FedSpam within the broader landscape of privacy-preserving machine learning and spam detection.

% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=\linewidth]{Figures/fedspam.png}
%   \caption{Fedspam word importance explained for classification \citep{sidhpura2023_fedspam:}}
%   \label{fig:fedspam}
% \end{figure*}

%While specific limitations are not explicitly outlined in the text, the paper details the use of the British English SMS Corpora dataset without providing a direct link. The methodology section covers federated learning, local model training, and server-side model aggregation, showcasing the innovative approach.  The best-performing algorithm, DistilBERT, attains a remarkable 98\% accuracy, though F1 score details are not explicitly mentioned. Additionally, SHapley Additive exPlanations (SHAP) is used for the global model, visualizing influential words in SMS and their impact on predictions. Figure \ref{fig:fedspam} illustrates this from the paper.


%Karhani et al. \citep{karhani_phishing_2023} also tried to explain the feature importance in their work introducing a hybrid machine learning model for phishing and smishing detection, employing domain features and Natural Language Processing (NLP) techniques, and integrated with MISP (Malware Information Sharing Platform) for the storage of flagged phishing domains. Trained and tested on datasets from TELUS Corp. and publicly available data, the model achieves an impressive accuracy of 99.40\% and an F1 score exceeding 99\%. The hybrid model combines a domain checker and NLP checker, with the domain checker excelling in classifying phishing domains. The NLP checker corrects the domain checker in 69.35\% of cases, though it struggles with generalization to TELUS's confirmed phishing dataset. The paper emphasizes the rising threat of phishing during the Covid-19 pandemic and proposes a comprehensive solution: a Machine Learning-based tool for real-time phishing and smishing detection, seamlessly integrated with MISP. The proposed model's robustness is highlighted by its accuracy and F1 score, and the paper shows feature engineering, the decision tree model's performance, and the tool's architecture, illustrated by figures. The work addresses the urgent need for a multifaceted detection tool and contributes a highly accurate solution to the cybersecurity domain and also provides feature importance (shown in figure \ref{fig:feature_importance}) to detect smishing messages.

% \begin{figure}[ht]
%   \centering
%   \includegraphics[width=\linewidth]{Figures/feature_importance.png}
%   \caption{Feature importance by the model \citep{karhani_phishing_2023}}
%   \label{fig:feature_importance}
% \end{figure}

% New table 5





%\footnote{In table 7, UCI machine learning SMS spam collection, Almeida spam dataset and UCI machine learning repository these threee datasets are same.}

%(\footnote{Sir, Ebbu2017 dataset is actually for core phishing url not for smishing and the paper [29] is itself a survey.})

%{\color{red}
%This section provides a comparative analysis of key performance metrics across various papers addressing smishing detection. We have added the compassion table for preparing the concise information for those collected research works. Because of the extensive information, we have separated the tables into four parts. Tables 2 to 6 show the key ideas with strengths and weaknesses reviewed by us. Notably, the surveyed studies employ diverse methodologies, including rule-based systems, machine learning models, and hybrid approaches, to combat the evolving tactics of smishing attackers. We have also summarized and compared the achieved results in terms of the dataset used, best model, accuracy, F1 score shown in table \ref{tab:result_sum} 
%\footnote{{\color{blue} Total publicly available datasets are UCI machine learning SMS spam collection, British English SMS, NUS SMS Corpus and Smishtank Dataset...Table 7 should be updated accordingly}}.

%Papers incorporating hybrid models, combining domain and Natural Language Processing (NLP) features, consistently report high accuracy rates exceeding 99\%. The integration of Support Vector Classifier (SVC) and decision tree models is prevalent, showcasing the effectiveness of combining diverse approaches.

%Studies leveraging continual learning techniques exhibit notable advantages in sustaining detection performance over time. A tolerable deterioration of 2.45\% in accuracy, as reported in one paper, outperforms traditional models, which experience more significant declines.

%Research focusing on content and URL analysis, particularly for smishing SMS, demonstrates precision rates above 98\%. Techniques such as Term Frequency-Inverse Document Frequency (TF-IDF) weighting frameworks contribute to the identification of rare words, enhancing detection accuracy.
%Machine Learning-Based Approaches:

%Machine learning-based models, ranging from Naive Bayes to Random Forest and Support Vector Machines, consistently achieve accuracy rates exceeding 99\%. Noteworthy is the emphasis on user involvement, allowing users to make decisions based on analysis results.

%Rule-based systems, employed in the context of mobile applications, showcase promising results in intercepting and classifying SMS messages. The user-centric approach of deciding whether to retain or discard messages contributes to personalized security.

%\footnote{this red texts are not contextual here, these are old texts which needs to be replaced to deleted if these are addressed in other section}

==> result_comparison.tex <==
\begin{table*}[t]
\caption{Analysis of Existing Models and Their Performance Evaluations}
\label{tab:result_sum}
\resizebox{\textwidth}{!}{
\begin{tabular}{rllllr}
\toprule
 SL &              Reference &                                      Datasets Used &                               Best Algorithm Model & Accuracy &  F1 Score \\
\midrule
  1 &     AKANDE et al, 2023 \citep{smsprotect_akande} &         UCI machine learning SMS spam collection.  &                              Naive Bayes algorithm &   0.9629 &       - \\
  2 &   ALKHALIL et al, 2021 \citep{phishing_comp_study_alkhalil} &                                                - &                                                - &      - &       - \\
  3 &    BOUKARI et al, 2021 \citep{mldetect_smishing_frauds_boukari}& Private &                                      Random Forest &      - &       - \\
  4 &       EJAZ et al, 2023 \citep{life_long_phsising_ejaz}&                                           Private &                      Continual Learning (LWF, EWC) &  94 (TP) &       - \\
  5 &   GHOURABI et al, 2021 \citep{smdetector_ghourabi}&                                            Private &                                            BERT-FC &   0.9963 &    0.9558 \\
  6 &    HOSSAIN et al, 2022 \citep{spam_filtering_cnn_lstm_hossain}&         UCI machine learning SMS spam collection.  &                                           CNN-LSTM &    0.984 &    0.9800 \\
  7 &       JAIN et al, 2022 \citep{content_url_analysis_jain}& Almeida spam dataset and Private dataset combination &                                     Neural Network &   0.9903 &       - \\
  8 &    KARHANI et al, 2023 \citep{karhani_phishing_2023}& Multiple anonymized datasets from TELUS Corporation and two from literature & Hybrid machine learning model &    0.994 &    0.9900 \\
  9 &     MISHRA et al, 2022 \citep{smishing_detector_security_model_mishra_2020}& Dataset from Literature &                                       Naive Bayes  &   0.9629 &       - \\
 10 &     MISHRA et al, 2022 \citep{implement_smishing_detector_mishra_2022}& Real-time smishing messages. Almedia spam dataset. Screenshots from Pinterest &                                     Neural Network &    0.974 &    0.8672 \\
 11 &     MISHRA et al, 2023 \citep{dsmish_mishra_2023}&                                            Private &             Multilayer Perceptron Back Propagation &   0.9793 &       - \\
 12 &    NEUPANE et al, 2015 \citep{multi_modal_neupane}&                                                - &                                                - &      - &       - \\
 13 &     RAHMAN et al, 2022 \citep{user_really_respond_rahman}&                                                - &                                                - &      - &       - \\
 14 &         SIDDIQI et al. \citep{a_study_psy_siddiqi}& Ebbu2017. Secondary online sources  &                                                - &      - &       - \\
 15 &      TIMKO et al, 2023 \citep{commerial_anti_smishing_timko}& UCI machine learning SMS spam collection and Private &                                                - &      - &       - \\
 16 & NAHAPETYAN et al, 2023 \citep{on_phishing_tactics_nahapetyan2023sms}&                                            Private &                                                - &      - &       - \\
 17 &   SIDHPURA et al, 2023 \citep{sidhpura2023_fedspam:}& British English SMS Corpora &                                         DistilBERT &     0.98 &       - \\
 18 & GOEL et al., 2018 \citep{goel2018smishing} & Lingo dictionary &  Naïve Bayesian algorithm & - & - \\
 19 & MISHRA et al. 2019 \citep{mishra2019content} & NUS SMS Corpus & Machine Learning algorithm & - & - \\
 20 & ULFATH et al., 2022 \citep{ulfath2022detecting} & UCI machine learning repository & Support vector machine (SVM) & 0.9839 & 0.9908 \\
 21 & BLANCAFLOR et al. 2021 \citep{blancaflor2021let} & Private & - & - & - \\
 22 & SONOWAL, 2020 \citep{sonowal2020detecting} & UCI Machine Learning Repository & Kendall rank correlation & 0.9840 & 0.9397 \\
 23 & NJUGUNA et al., 2021 \citep{njuguna2021model} & Private & Naive Bayes Classifier & 0.9420 & 0.9700 \\
 24 & KANAOKA et al., 2023 \citep{kanaoka2023beyond} & - & Google’s ML Kit API & 0.8519 & - \\
 25 & GHOURABI et al., 2020 \citep{ghourabi2020hybrid} & UCI machine learning repository & CNN-LSTM & 0.9837 & 0.9148 \\
 26 & CLASEN et al., 2021 \citep{clasen2021friend} & Private & - & - & - \\
 27 & SEO et al., 2024 \citep{seo2024device} & Korean Internet and Security Agency (KISA) & Char-CNN & 0.9960 & 0.9944 \\
 28 & TIMKO et al., 2024 \citep{timko2024smishing} & Smishtank Dataset & - & - & - \\
 
\bottomrule
\end{tabular}

}
\end{table*}

\footnote{In table 7, UCI machine learning SMS spam collection, Almeida spam dataset and UCI machine learning repository these threee datasets are same.}

(\footnote{Sir, Ebbu2017 dataset is actually for core phishing url not for smishing and the paper [29] is itself a survey.})


This section provides a comparative analysis of key performance metrics across various papers addressing smishing detection. We have added the compassion table for preparing the concise information for those collected research works. Because of the extensive information, we have separated the tables into four parts. Tables 2 to 6 show the key ideas with strengths and weaknesses reviewed by us. Notably, the surveyed studies employ diverse methodologies, including rule-based systems, machine learning models, and hybrid approaches, to combat the evolving tactics of smishing attackers. We have also summarized and compared the achieved results in terms of the dataset used, best model, accuracy, F1 score shown in table \ref{tab:result_sum} \footnote{{\color{blue} Total publicly available datasets are UCI machine learning SMS spam collection, British English SMS, NUS SMS Corpus and Smishtank Dataset...Table 7 should be updated accordingly}}.

Papers incorporating hybrid models, combining domain and Natural Language Processing (NLP) features, consistently report high accuracy rates exceeding 99\%. The integration of Support Vector Classifier (SVC) and decision tree models is prevalent, showcasing the effectiveness of combining diverse approaches.

Studies leveraging continual learning techniques exhibit notable advantages in sustaining detection performance over time. A tolerable deterioration of 2.45\% in accuracy, as reported in one paper, outperforms traditional models, which experience more significant declines.

Research focusing on content and URL analysis, particularly for smishing SMS, demonstrates precision rates above 98\%. Techniques such as Term Frequency-Inverse Document Frequency (TF-IDF) weighting frameworks contribute to the identification of rare words, enhancing detection accuracy.
Machine Learning-Based Approaches:

Machine learning-based models, ranging from Naive Bayes to Random Forest and Support Vector Machines, consistently achieve accuracy rates exceeding 99\%. Noteworthy is the emphasis on user involvement, allowing users to make decisions based on analysis results.

Rule-based systems, employed in the context of mobile applications, showcase promising results in intercepting and classifying SMS messages. The user-centric approach of deciding whether to retain or discard messages contributes to personalized security.


\begin{table*}[!t]
    \centering
    \caption{Summary of Publicly Available SMS Phishing Related Datasets}
    \resizebox{0.999\textwidth}{!}{
    \begin{tabular}{*{3}{c}|*{9}{c}|*{3}{c}}
        \hline
        \multirow{2}{*}{Dataset} & \multirow{2}{*}{Format} & \multirow{2}{*}{Labeled} & \multicolumn{3}{c}{\# Instances} & \multicolumn{3}{c}{Avg. $\left| message \right|$} & \multicolumn{3}{c|}{Std. $\left| message \right|$}  & \multirow{2}{*}{\#URL Message} & \multirow{2}{*}{\#Phn Message} & \multirow{2}{*}{\#Email Message}\\
        \cline{4-12}
         & & & full & ham & spam & full & ham & spam & full & ham & spam\\
        \hline

        British & .doc & yes & 875 & 875 & 875 & 106.82 & 78.89 & 136.4 & 46.78 & 42.34 & 30.13 & 99 (11.31\%)& 176 (20.11\%) & 9 (1.03\%)\\

        NUS & .json & no & 55835 & - & - & 52.01 & - & - & 54.17 & - & - & 3433 (6.15\%)& 52 (0.09\%) & 28 (0.05\%)\\

        UCI & .txt & yes & 5574 & 5574 & 5574 & 80.48 & 71.47 & 138.68 & 59.84 & 58.32 & 28.85 & 495 (8.88\%)& 336 (6.03\%) & 16 (0.29\%)\\

        Smishtank & .csv & no & 1091 & - & - & 176.96 & - & - & 121.28 & - & - & 938 (85.98\%)& 38 (3.48\%) & 6 (0.55\%)\\
        \hline
    \end{tabular}
    \label{table:dat_details}
    }
\end{table*}

\footnote{add the label data percentage for the labeled data in table 8}

==> thematic_organization.tex <==



% \begin{figure*}
%   \centering
%   \begin{tikzpicture}[>=Stealth, node distance=1.5cm, every node/.style={text width=2.5cm, align=center, rectangle, draw, minimum height=1cm}]

%     % Nodes
%     \node (smishing) {Smishing Research and Detection};
    
%     \node[below=of smishing, yshift=-2.0cm] (study) {Study/Rule Based};
    
%     \node[below=of study, xshift=-1.5cm] (userstudy) {User study};
%     \node[below=of study, xshift=1.5cm] (psychstudy) {Psych Study};
    
%     \node[below=of smishing, xshift=4.5cm, yshift=-0.5cm] (msganalysis) {Message Analysis};
    
%     \node[below=of msganalysis, yshift=-0.5cm] (contentanalysis) {Content Analysis};
    
%     \node[below=of contentanalysis, xshift=-3.5cm, yshift=-1.5cm] (classicml) {Classic ML};
%     \node[below=of contentanalysis, xshift=-0.5cm, yshift=-1.5cm] (deeplearning) {Deep Learning};
    
%     \node[below=of msganalysis, xshift=3.0cm, yshift=-0.5cm] (urlanalysis) {URL Analysis};
    
%     \node[below=of urlanalysis, xshift=-1.5cm] (lexicalfeatures) {Lexical Features};
%     \node[below=of urlanalysis, xshift=1.5cm] (hostfeatures) {Host-based Features};
    
%     \node[below=of smishing, xshift=-4.5cm, yshift=-0.5cm] (modelexplain) {Model Explainability};
    
%     \node[below=of modelexplain, xshift=-1.5cm] (localapprox) {Local Approximations};
%     \node[below=of modelexplain, xshift=1.5cm] (globalimportance) {Global Feature Importance};
    
%     % Arrows
%     \draw[->] (smishing) -- (study);
%     \draw[->] (study) -- (userstudy);
%     \draw[->] (study) -- (psychstudy);
%     \draw[->] (smishing) -- (msganalysis);
%     \draw[->] (msganalysis) -- (contentanalysis);
%     \draw[->] (contentanalysis) -- (classicml);
%     \draw[->] (contentanalysis) -- (deeplearning);
%     \draw[->] (msganalysis) -- (urlanalysis);
%     \draw[->] (urlanalysis) -- (lexicalfeatures);
%     \draw[->] (urlanalysis) -- (hostfeatures);
%     \draw[->] (smishing) -- (modelexplain);
%     \draw[->] (modelexplain) -- (localapprox);
%     \draw[->] (modelexplain) -- (globalimportance);
    
%   \end{tikzpicture}
%   \caption{Smishing research and detection literature category}
%   \label{fig:category_smishing}
% \end{figure*}

\begin{figure*}[h]
  \centering
  \includegraphics[width=\linewidth]{Figures/thematic_org.png}
  \caption{Thematic Diagram of Smishing Research.}
  \label{fig:thematic-diagram}
\end{figure*}

\footnote{deep learning is not inlcuded in figure 1 in the present version...need to address!}

{\footnote{\color{blue} adding a timeline image of history of smishing}}
The literature motivates us towards smishing research and detection techniques into three main approaches:

% \begin{itemize}
%     \item Study/ Rule Based Research works - Analyzes rule based systems, SMS phishing related user studies, psychological patterns with smishing attacks
    
%     \item Content analysis - Analyzes message text using Classical ML and deep learning

%     \item URL analysis - Identifies malicious URLs in messages using lexical or host features

%     \item Model explainability - Generates local or global explanations for model predictions

% \end{itemize}

\begin{itemize}
    \item Smishing Attacks - This branch explores the different ways attackers use smishing to achieve their goals.
    
    \item Smishing Detection - This branch examines the various approaches used to identify and prevent smishing attempts.

    \item Smishing countermeasure - This branch outlines the strategies employed to mitigate the risks associated with smishing.

\end{itemize}


We have gathered Scopus-indexed articles for this literature review with good impact factor journals or conferences. The prior arts we are discussing in this section follow this tree of research problems and solution methodologies. The key branches are also shown in figure \ref{fig:thematic-diagram}:

\begin{itemize}
    \item Smishing Attacks
        \begin{itemize}
            \item Types of Smishing Attacks: Explains the various objectives attackers have, such as stealing credentials, distributing malware, or directly obtaining financial gain \citep{on_phishing_tactics_nahapetyan2023sms}.
            \item Smishing Techniques: Details the manipulative tactics used by attackers to trick victims, like social engineering, urgency creation, and sender spoofing \citep{phishing_comp_study_alkhalil}.
            \item Impact of Smishing: Highlights the potential consequences for victims who fall prey to smishing attacks, including financial loss, identity theft, and data breaches \citep{clasen2021friend}.
        \end{itemize}
    \item Smishing Detection
        \begin{itemize}
            \item Rule-based Detection: Explains traditional methods that rely on predefined rules to flag suspicious messages based on keywords, URLs, or sender patterns \citep{smsprotect_akande}.
            
            \item Machine Learning Techniques: Discusses the use of advanced algorithms (supervised learning, anomaly detection) to analyze messages and identify potential smishing attempts with greater accuracy \citep{commerial_anti_smishing_timko}.

            \item User Awareness and Education: Emphasizes the importance of educating users to recognize red flags and develop safe practices for interacting with SMS messages \citep{blancaflor2021let}.
        
        \end{itemize}
    
    \item Smishing countermeasure

        \begin{itemize}            
            \item Secure Mobile Technologies: Explores the use of security features on mobile devices, such as SMS filtering and two-factor authentication, to prevent smishing attacks from succeeding \citep{a_study_psy_siddiqi}.
            
            \item User Behavioral Training: Highlights the importance of training users to identify smishing attempts through simulations and education on safe browsing habits \citep{clasen2021friend}.

            \item Law Enforcement and Regulatory Efforts: Discusses the role of law enforcement in tracking cybercriminals and the development of regulations to protect consumers from smishing threats \citep{faklaris2024mitigating}.
        
        \end{itemize}

\end{itemize}

By understanding the various types of smishing attacks (Branch 1), the methods used to detect them (Branch 2), and the available countermeasures (Branch 3), we can effectively combat this growing cybersecurity threat. This comprehensive approach that combines technical detection methods with user awareness and education, alongside law enforcement efforts, strengthens our defenses against smishing scams and protects individuals from potential financial loss and identity theft.

Moreover, in table \ref{tab:method_sum} we have shown all the works' methodology according to our thematic organization to show the diversity of the research work we chose to survey.
